Seeing is Believing: A Unified Model for Consistency and Isolation via States

This paper introduces a unified model of consistency and isolation that minimizes the gap between how these guarantees are defined and how they are perceived. Our approach is premised on a simple observation: applications view storage systems as black-boxes that transition through a series of states, a subset of which are observed by applications. For maximum clarity, isolation and consistency guarantees should be expressed as constraints on those states. Instead, these properties are currently expressed as constraints on operation histories that are not visible to the application. We show that adopting a state-based approach to expressing these guarantees brings forth several benefits. First, it makes it easier to focus on the anomalies that a given isolation or consistency level allows (and that applications must deal with), rather than those that it proscribes. Second, it unifies the often disparate theories of isolation and consistency and provides a structure for composing these guarantees. We leverage this modularity to apply to transactions (independently of the isolation level under which they execute) the equivalence between causal consistency and session guarantees that Chockler et al. had proved for single operations. Third, it brings clarity to the increasingly crowded field of proposed consistency and isolation properties by winnowing spurious distinctions: we find that the recently proposed parallel snapshot isolation introduced by Sovran et al. is in fact a specific implementation of an older guarantee, lazy consistency (or PL-2+), introduced by Adya et al.

==> causal.tex <==
\subsection{Causal consistency and Session Guarantees}


\begin{lemma}
	\label{sfolemma}
	For any $\mathcal{T}'$ that $\mathcal{T}' \subseteq \mathcal{T}$, $\prereadmath{e}{\mathcal{T}'} \Leftrightarrow \forall t \in \mathcal{T}': \forall o \in \Sigma_t: \sfomath{o} \xrightarrow{+} s_{t}$.
\end{lemma}

\begin{proof}
	($\Rightarrow$) Given $\prereadmath{e}{\mathcal{T}'}$, by definition we have $ \forall t \in \mathcal{T}', \forall o \in \Sigma_t$, $\RSmath{o} \neq \emptyset$.
	
	If $o= r(k,v)$,  $\RSmath{o} = \{s \in \mathcal{S}_e | 
	s \xrightarrow{*} s_p \wedge\big ( (k,v) \in s \vee (\exists w(k,v) \in \Sigma_t: w(k,v) \xrightarrow{to} r(k,v)) \big)\}$.
	\begin{enumerate}
		\item if $\exists w(k,v) \in \Sigma_t: w(k,v) \xrightarrow{to} r(k,v)$, $\RSmath{o} = \{s \in \mathcal{S}_e | s \xrightarrow{*} s_p\}$, therefore $\sfomath{o} = s_0 \xrightarrow{+} s_t$
		\item if $\not\exists w(k,v) \xrightarrow{to} r(k,v)$, by $\RSmath{o} \neq \emptyset$, there exists $s \in \mathcal{S}_e$, s.t. $s \xrightarrow{*} s_p \wedge (k,v) \in s$. Since $\sfomath{o}$ is first such $s$, we have $\sfomath{o} \xrightarrow{*}s_p \rightarrow s_t$, i.e. $\sfomath{o} \xrightarrow{+} s_t$.
	\end{enumerate}
	
	If $o=w(k,v)$, then $\RSmath{o} = \{s \in \mathcal{S}_e | 
	s \xrightarrow{*} s_p\}$, therefore $\sfomath{o} = s_0 \xrightarrow{+} s_t$.
	
	Therefore we have proved that $\forall t \in \mathcal{T}': \forall o \in \Sigma_t: \sfomath{o} \xrightarrow{+} s_{t}$.
	
	($\Leftarrow$) Given $\forall t \in \mathcal{T}': \forall o \in \Sigma_t: \sfomath{o} \xrightarrow{+} s_{t}$, since $\sfomath{o} \in \RSmath{o}$, therefore $\forall t \in \mathcal{T}': \forall o \in \Sigma_t: \RSmath{o} \neq \emptyset$, i.e. $\prereadmath{e}{\mathcal{T}'}$ holds.
\end{proof}

\begin{lemma}
	\label{prereadlemma}
	For any $\mathcal{T}'$ that $\mathcal{T}' \subseteq \mathcal{T}$, $\prereadmath{e}{\mathcal{T}} \Rightarrow \prereadmath{e}{\mathcal{T}'}$.
\end{lemma}

\begin{proof}
	Given $\prereadmath{e}{\mathcal{T}}$, by definition we have $ \forall t \in \mathcal{T}, \forall o \in \Sigma_t$, $\RSmath{o} \neq \emptyset$. Since $\mathcal{T}' \subseteq \mathcal{T}$, $\forall t \in \mathcal{T}' \Rightarrow \forall t \in \mathcal{T}$, therefore we have $ \forall t \in \mathcal{T}', \forall o \in \Sigma_t$, $\RSmath{o} \neq \emptyset$, i.e. $\prereadmath{e}{\mathcal{T}'}$.
\end{proof}


\begin{theorem}
	A storage system satisfies causal consistency if and only if it satisfies the four session guarantees: Read-My-Writes (RMW), Monotonic Reads (MR), Monotonic Writes (MW), Write-Follow-Reads(WFR).
\end{theorem}


\begin{proof}
	
	($\Rightarrow$) First we prove the direction that Causal Consistency (CC) $\Rightarrow$ RMW, MR, MW, WFR.
	
	Given the storage system satisfies causal consistency, i.e. $\forall se \in SE: \exists e:  \forall t \in T_{se} : \sessionmath{CC}{se}{t}{e} $, where $ \sessionmath{CC}{se}{t}{e} \equiv   \prereadmath{e}{\mathcal{T}} \wedge \ircmath{e}{t} \wedge (\forall o \in \Sigma_t: \forall t' \xrightarrow{se} t:  s_{t'} \xrightarrow{*} sl_o) \wedge (\forall se' \in SE: \forall t_i \xrightarrow{se'} t_j: s_{ti} \xrightarrow{*} s_{tj})$. 
	
	For any $se \in SE$, consider the execution $e$, s.t. $\forall t \in T_{se}: \sessionmath{CC}{se}{t}{e} $:
	
	\begin{description}
		\item[CC $\Rightarrow$ RMW]: Since $e$ satisfies $\forall t \in T_{se}: \forall o \in \Sigma_t: \forall t' \xrightarrow{se} t:  s_{t'} \xrightarrow{*} sl_o$ by definition of $ \sessionmath{CC}{se}{t}{e}$, by weakening the statement, we have $e$ satisfies $\forall o \in \Sigma_t: \forall t'\xrightarrow{se} t:\mathcal{W}_{t'} \neq \emptyset \Rightarrow s_{t'} \xrightarrow{*}sl_o$. 
		Since $e$ also satisfies $\prereadmath{e}{\mathcal{T}}$ and $\mathcal{T}_{se} \subseteq \mathcal{T}$, by lemma \ref{prereadlemma}, $e$ satisfies $\prereadmath{e}{\mathcal{T}_{se}}$. 
		Therefore $e$ satisfies $\prereadmath{e}{\mathcal{T}_{se}} \wedge \forall o \in \Sigma_t: \forall t'\xrightarrow{se} t:\mathcal{W}_{t'} \neq \emptyset \Rightarrow s_{t'} \xrightarrow{*}sl_o$, hence we proved $\forall se \in SE: \exists e:  \forall t \in T_{se} : \sessionmath{RMW}{se}{t}{e}$.
		
		\item[CC $\Rightarrow$ MW]: 
		Since $e$ satisfies $\forall se' \in SE: \forall t_i \xrightarrow{se'} t_j: s_{t_i} \xrightarrow{+} s_{t_j}$ by definition of $ \sessionmath{CC}{se}{t}{e}$, by weakening the statement, we have $e$ satisfies $\forall se' \in SE: \forall t_i' \xrightarrow{se'} t_j: (\mathcal{W}_{t_i} \neq \emptyset \wedge
		\mathcal{W}_{t_j} \neq \emptyset) \Rightarrow s_{t_i} \xrightarrow{+} s_{t_j} $. 
		Since $e$ also satisfies $\prereadmath{e}{\mathcal{T}}$ and $\mathcal{T}_{se} \subseteq \mathcal{T}$, by lemma \ref{prereadlemma}, $e$ satisfies $\prereadmath{e}{\mathcal{T}_{se}}$. 
		Therefore $e$ satisfies $\prereadmath{e}{\mathcal{T}_{se}} \wedge \forall se' \in SE: \forall t_i' \xrightarrow{se'} t_j: (\mathcal{W}_{t_i} \neq \emptyset \wedge	\mathcal{W}_{t_j} \neq \emptyset) \Rightarrow s_{t_i} \xrightarrow{+} s_{t_j} $, hence we proved $\forall se \in SE: \exists e:  \forall t \in T_{se} : \sessionmath{MW}{se}{t}{e}$.

		\item[CC $\Rightarrow$ MR]: By definition of $ \sessionmath{CC}{se}{t}{e}$, $e$ satisfies $\forall t \in T_{se}: \forall o \in \Sigma_t: \forall t' \xrightarrow{se} t:  s_{t'} \xrightarrow{*} sl_o$.  
		Since $e$ also satisfies $\prereadmath{e}{\mathcal{T}}$, from lemma \ref{sfolemma}, we have $\forall t' \in \mathcal{T}: \forall o' \in \Sigma_{t'}: \sfomath{o'} \xrightarrow{+} s_{t'}$. 
		Combining the two statement, we have $\forall o \in \Sigma_t: \forall t_i \xrightarrow{se} t: \forall o' \in \Sigma_{t'}: \sfomath{o'} \xrightarrow{*} s_{t'} \xrightarrow{*} \slomath{o} $, i.e. $\sfomath{o'} \xrightarrow{*}  \slomath{o}$. 
		Again from $\prereadmath{e}{\mathcal{T}}$ and $\mathcal{T}_{se} \subseteq \mathcal{T}$, by lemma \ref{prereadlemma}, $e$ satisfies $\prereadmath{e}{\mathcal{T}_{se}}$. 
		From definition of $ \sessionmath{CC}{se}{t}{e}$, $e$ satisfies $\ircmath{e}{t}$.
		Therefore $e$ satisfies 
		$\prereadmath{e}{\mathcal{T}_{se}} \wedge \ircmath{e}{t} \wedge \forall o \in \Sigma_t: \forall t'\xrightarrow{se}t: \forall o' \in \Sigma_{t'}: sf_{o'}\xrightarrow{*}sl_o $, hence we proved $\forall se \in SE: \exists e:  \forall t \in T_{se} : \sessionmath{MR}{se}{t}{e}$.
		
		\item[CC $\Rightarrow$ WFR]: By definition of $ \sessionmath{CC}{se}{t}{e}$, $e$ satisfies $\forall se' \in SE: \forall t_i \xrightarrow{se'} t_j: s_{t_i} \xrightarrow{+} s_{t_j}$.  
		Since $e$ also satisfies $\prereadmath{e}{\mathcal{T}}$, from lemma \ref{sfolemma}, we have $\forall t_i \in \mathcal{T}: \forall o_i \in \Sigma_{t_i}: \sfomath{o_i} \xrightarrow{+} s_{t_i}$. 
		Combining the two statement, we have $\forall se' \in SE: \forall t_i\xrightarrow{se'}t_j: \forall o_i \in \Sigma_{t_i}: sf_{o_i} \xrightarrow{*} s_{t_i} \xrightarrow{+} s_{t_j} $, i.e. $sf_{o_i} \xrightarrow{+} s_{t_j} $. 
		By weakening the statement, we have $\forall se' \in SE: \forall t_i\xrightarrow{se'}t_j: \forall o_i \in \Sigma_{ti}:\mathcal{W}_{t_j} \neq \emptyset \Rightarrow sf_{o_i} \xrightarrow{+} s_{t_j} $.
		Again from $\prereadmath{e}{\mathcal{T}}$ and $\mathcal{T}_{se} \subseteq \mathcal{T}$, by lemma \ref{prereadlemma}, $e$ satisfies $\prereadmath{e}{\mathcal{T}_{se}}$. 
		Therefore
		$e$ satisfies 
		$\prereadmath{e}{\mathcal{T}} \wedge \forall se' \in SE: \forall t_i\xrightarrow{se'}t_j: \forall o_i \in \Sigma_{ti}:\mathcal{W}_{t_j} \neq \emptyset \Rightarrow sf_{o_i} \xrightarrow{+} s_{t_j} $, hence we proved $\forall se \in SE: \exists e:  \forall t \in T_{se} : \sessionmath{WFR}{se}{t}{e}$.
				
	\end{description}
	
	($\Leftarrow$) Now we prove the other direction:
	
	Let $\mathcal{G} = \{RMW,MR,MW,WFR \}$, we want to prove that $\forall se \in SE :\exists e: \forall t \in T_{se} :\sessionmath{\mathcal{G}}{se}{t}{e} 
	\Rightarrow \forall se \in SE : \exists e :  \forall t \in T_{se}: \sessionmath{CC}{se}{t}{e}$
	
	We prove the statement by proving that for any session $se$, given the execution $e$ that $\forall t \in T_{se} :\sessionmath{\mathcal{G}}{se}{t}{e} $, we can construct an execution $e'$, such that $\forall t \in T_{se}: \sessionmath{CC}{se}{t}{e'}$.
	
	We construct $e'$ as following: First, we apply all the transactions $t$ that $\mathcal{W}_t \neq \emptyset$ in the same order as in $e$. We denote the states created by applying $t$ in $e$ and $e'$ as $s_{e,t}$ and $s_{e',t}$ respectively. Then we claim that $\forall t \in \mathcal{T} \wedge \mathcal{W}_t \neq \emptyset:  (k,v) \in s_{e,t} \Leftrightarrow (k,v) \in s_{e',t}$,  denoted as $s_{e,t} \equiv s_{e',t}$. The claim is true because the update transactions are applied in $e'$ the same order as $e$, $e$ is therefore only different from $e'$ on that $e$ also applies read-only transactions, however read-only transactions does not change the value of keys. 
	
 Second, we consider each read-only transaction $t$ in the order specified by $e$, however, we select the parent state for $t$ to be $\max\{\max_{o \in \Sigma_t}\{\sfomath{o}\}, s_{t_{-1}}\}$, where $ t_{-1}$ denotes the transaction that directly precedes $t$ in a session. Since we consider session order to be a total order, there is at most one such transaction. If no such transaction exists, $s_{t_{-1}} = s_0$. Note that since $t$ is a read-only transaction, applying read-only transactions does not change the value of states, therefore it still holds that $\forall t \in \mathcal{T} \wedge \mathcal{W}_t \neq \emptyset: s_{e,t} \equiv s_{e',t}$.
 	
 	
 	\begin{clm}
 		$\prereadmath{e'}{\mathcal{T}}$ is true.
 		\label{claim:pretrue}
 	\end{clm}
 	\begin{proof}
 		For any the update transaction $t$:
 		\begin{description}
 			\item[$o = r(k,v) \in \Sigma_t$] If $\sfomath{o}$ exists, then it must created by applying an update transaction $t' \in \mathcal{T}$ which updates key $k$ with value $v$, i.e. $\sfomath{o} = s_{t'}$. Since $e$ satisfies $\prereadmath{e}{\mathcal{T}}$ as required in $WFR$, by lemma \ref{sfolemma}  $s_{t'} \xrightarrow{+} s_{t}$ in $e$. And since we apply update transactions in $e'$ the same order as $e'$, therefore $s_{t'} \xrightarrow{+} s_{t}$ in $e'$, i.e. $\sfomath{o} \xrightarrow{+} s_{t}$ in $e'$.
 			
 			\item[$o=w(k,v)\in \Sigma_t$] Since for write operations, $\sfomath{o} = s_0$, then trivially $\sfomath{o} \xrightarrow{+} s_t$ in $e'$.
 		\end{description} 
 		
 		For any read-only transaction $t$:
 		Since $s_p(t) = \max\{\max_{o \in \Sigma_t}\{\sfomath{o}\}, s_{t_{-1}}\}$, we have $\forall o \in \Sigma_t, s_p(t) \geq \sfomath{o}$, therefore $\sfomath{o} \xrightarrow{*} s_p(t) \rightarrow s_t$, i.e. $\forall o \in \Sigma_t:\sfomath{o} \xrightarrow{+} s_t$.
 		
 		Therefore $\forall t \in \mathcal{T}: \forall o \in \Sigma_t: \sfomath{o} \xrightarrow{+} s_{t}$ in $e'$, by lemma \ref{sfolemma}, $\prereadmath{e'}{\mathcal{T}}$ holds.
 	\end{proof}
 	
 	\begin{clm}
 		$\forall t \in T_{se} :\sessionmath{MW}{se}{t}{e'}  \wedge \sessionmath{WFR}{se}{t}{e'} $.
 		\label{claim:MWWFR}
 	\end{clm}
 	
 	\begin{proof}
 		
 		Since we have $\forall t \in T_{se} :\sessionmath{MW}{se}{t}{e}  \wedge \sessionmath{WFR}{se}{t}{e} $, now we consider $e'$.
 		
 	
 			\begin{description}
 				\item[MW] In any $se' \in SE$, consider any $t_i, t_j$ that $t_i \xrightarrow{se'} t_j$, and $\mathcal{W}_{t_i} \neq \emptyset \wedge \mathcal{W}_{t_j} \neq \emptyset$. Since $e$ satisfies $\forall t \in T_{se} :\sessionmath{MW}{se}{t}{e'} $, we have $s_{e,t_i} \xrightarrow{+} s_{e,t_j} $.  Since $t_i$ and $t_j$ are update transactions and are therefore applied in $e'$ the same order in $e$, hence we have $s_{e',t_i} \xrightarrow{+} s_{e',t_j}$. We have proved that $\prereadmath{e'}{\mathcal{T}}$ and $\mathcal{T}_{se} \subseteq \mathcal{T}$, by Lemma~\ref{prereadlemma}, we have $\prereadmath{e'}{\mathcal{T}_{se}}$ Then we claim that $\prereadmath{e'}{\mathcal{T}_{se}} \wedge \forall se' \in SE: \forall t_i \xrightarrow{se'} t_j: (\mathcal{W}_{t_i} \neq \emptyset \wedge
 				\mathcal{W}_{t_j} \neq \emptyset) \Rightarrow s_{t_i} \xrightarrow{+} s_{t_j} $, i.e. $\forall t \in T_{se} :\sessionmath{MW}{se}{t}{e'}$.
 				
 				\item[WFR] Consider $\forall se' \in SE: \forall t_i\xrightarrow{se'}t_j: \forall o_i \in \Sigma_{t_i}:\mathcal{W}_{t_j} \neq \emptyset $, we want to prove that $sf_{o_i} \xrightarrow{+} s_{t_j} $:
 				
 				\begin{description}
 					\item[$o_i = r(k,v)$] If $\sfomath{o}$ exists, then it must created by applying an update transaction $t' \in \mathcal{T}$ which updates key $k$ with value $v$, i.e. $\sfomath{o_i} = s_{t'}$. Since $e$ satisfies $\forall t \in T_{se} :\sessionmath{WFR}{se}{t}{e'}$, we have $\sfomath{o_i} \xrightarrow{+} s_{t_j}$ in $e$, i.e. $s_{t'} \xrightarrow{+} s_{t_j}$ in $e$. And since we apply update transactions in $e'$ the same order as $e$, therefore $s_{t'} \xrightarrow{+} s_{t_j}$ in $e'$, i.e. $\sfomath{o_i} \xrightarrow{+} s_{t_j}$ in $e'$.
 					
 					\item[$o_i=w(k,v)$] Since for write operations, $\sfomath{o} = s_0$, then trivially $\sfomath{o_i} \xrightarrow{+} s_{t_j}$ in $e'$.
 				\end{description} 
 				Therefore we have proved that $\forall se \in SE :\forall t \in T_{se} :\sessionmath{WFR}{se}{t}{e'} $.
 			\end{description}
 	\end{proof}
 	
 	Now we want to prove that in $e'$, $\forall se' \in SE: \forall t_i \xrightarrow{se'} t_j: s_{t_i} \xrightarrow{+} s_{t_j}$ in two steps. 
 	
 	Given any session $se'$:
 	\begin{description}
 		\item[Step 1] Consider any $t_j \in \mathcal{T}_{se'} \wedge \mathcal{W}_{t_j} \neq \emptyset $, and each pair $(t_i,t_j)$ that $t_i \xrightarrow{se'} t_j$, we want to prove that $s_{t_i} \xrightarrow{+} s_{t_j}$:
 		\begin{enumerate}
 			\item For all $\mathcal{W}_{t_i} \neq \emptyset$, by Claim~\ref{claim:MWWFR}, $\forall t \in T_{se'} :\sessionmath{MW}{se'}{t}{e'}$, therefore $s_{t_i} \xrightarrow{+} s_{t_j}$ in $e'$.
 			
 			\item  Now we consider all the $t_i$ that $\mathcal{W}_{t_i} = \emptyset$, we prove $s_{t_i} \xrightarrow{+} s_{t_j}$ in $e'$ by induction:
 			
 			\begin{description}
 				\item[Base case] Consider the first read-only transaction $t_i$ in session $se'$, remember that we choose the parent state of a read-only transaction as $s_p(t_i) = \max\{\max_{o_i \in \Sigma_{t_i}}\{\sfomath{o_i}\}, s_{t_{i-1}}\}$, where $ t_{i-1}$ denotes the transaction that directly precedes $t_i$ in session $se'$. Therefore either $s_p(t_i) = \max_{o_i \in \Sigma_{t_i}}\{ \sfomath{o_i} \} $, or $s_{t_i} = s_{t_{i-1}} \wedge \mathcal{W}_{t_{i-1}} \neq \emptyset$.
 				
 				\begin{enumerate}
 					\item 	If $s_p(t_i) = \max_{o_i \in \Sigma_{t_i}}\{ \sfomath{o_i} \} $: By Claim~\ref{claim:MWWFR}, $\forall t \in T_{se} :\sessionmath{WFR}{se}{t}{e'}$, we have $\forall o_i \in \Sigma_{t_i}: \sfomath{o_i} \xrightarrow{+} s_{t_j}$ in $e'$, therefore $\max_{o_i \in \Sigma_{t_i}}\{ \sfomath{o_i} \} \xrightarrow{+} s_{t_j}$ in $e'$. Now we have $s_p(t_i)  \xrightarrow{+} s_{t_j}$ in $e'$, therefore $s_p(t_i) \rightarrow s_{t_i} \xrightarrow{*} s_{t_j}$ in $e'$.
 					
 					\item If $s_p({t_i}) = s_{t_{i-1}} \wedge \mathcal{W}_{t_{i-1}} \neq \emptyset$: Consider $(t_{i-1}, t_j)$, since we know that $t_{i-1} \xrightarrow{se'} t_i \xrightarrow{se'} t_j $, we have $ t_{i-1} \xrightarrow{se'} t_j$. Furthermore, we have the conditions that $\mathcal{W}_{t_{i-1}} \neq \emptyset \wedge \mathcal{W}_{t_j} \neq \emptyset$, therefore by Claim~\ref{claim:MWWFR},  $\forall t \in T_{se} :\sessionmath{MW}{se}{t}{e'}$, we have $ s_{t_{i-1}} \xrightarrow{+} s_{t_j}$. Now we have $s_p(t_i)  \xrightarrow{+} s_{t_j}$ in $e'$,  therefore $s_p(t_i) \rightarrow s_{t_i} \xrightarrow{*} s_{t_j}$. 
 				\end{enumerate}
 				
 				Since $t_i \xrightarrow{se'} t_j$, we have $t_i \neq t_j$, therefore $s_{t_i} \neq s_{t_j} \Rightarrow s_{t_i} \xrightarrow{+} s_{t_j}$. 
 				
 				
 				\item[Induction step] Assume that the k-th read-only transaction $t_i$ in $se'$, s.t. $t_i \xrightarrow{se'} t_j$, satisfies $\forall o \in \Sigma_t: s_{t_i} \xrightarrow{+} s_{t_j}$. Now we we consider the (k+1)-th read-only transaction $t_i'$ in $se'$, s.t. $t_i' \xrightarrow{se'} t_j$. Note that either $t_i$ directly precedes $t_i'$ in $se'$, or there exists an update transaction that directly precedes $t_i'$ in $se'$.
 				
 				Again either $s_p(t_i') = \max_{o_i' \in \Sigma_{t_i'}}\{ \sfomath{o_i'} \} $, or $s_{t_i'} = s_{t_{i-1}'}$, where $t_{i-1}'$ denotes the transaction directly precedes $t_i'$ in a session. Note that either $\mathcal{W}_{t'_{i-1}}= \emptyset \Rightarrow t_{i-1}'=t_i$  or $\mathcal{W}_{t'_{i-1}} \neq \emptyset$.
 				
 				\begin{enumerate}
 					\item 	If $s_p(t_i') = \max_{o_i' \in \Sigma_{t_i'}}\{ \sfomath{o_i'} \} $: By Claim~\ref{claim:MWWFR}, $\forall t \in T_{se} :\sessionmath{WFR}{se}{t}{e'}$, we have $\forall o_i' \in \Sigma_{t_i'}: \sfomath{o_i'} \xrightarrow{+} s_{t_j}$ in $e'$, therefore $\max_{o_i' \in \Sigma_{t_i'}}\{ \sfomath{o_i'} \} \xrightarrow{+} s_{t_j}$ in $e'$. Now we have $s_p(t_i')  \xrightarrow{+} s_{t_j}$ in $e'$, therefore $s_p(t_i') \rightarrow s_{t_i} \xrightarrow{*} s_{t_j}$ in $e'$.
 					
 					\item If $s_p{(t_i')} = s_{t_{i-1}'}$: Consider $(t_{i-1}', t_j)$, since we know that $t_{i-1}' \xrightarrow{se'} t_i' \xrightarrow{se'} t_j $, we have $ t_{i-1}' \xrightarrow{se'} t_j$. If $\mathcal{W}_{t_{i-1}'} \neq \emptyset $, we have the conditions that $\mathcal{W}_{t_{i-1}'} \neq \emptyset \wedge \mathcal{W}_{t_j} \neq \emptyset$, therefore by Claim~\ref{claim:MWWFR},  $\forall t \in T_{se} :\sessionmath{MW}{se}{t}{e'}$, we have $ s_{t_{i-1}'} \xrightarrow{+} s_{t_j}$, i.e. $s_p(t_i')  \xrightarrow{+} s_{t_j}$ in $e'$. If $\mathcal{W}_{t_{i-1}'} = \emptyset $, i.e. $t_{i-1}' = t_i$, therefore $s_p{(t_i')} = s_{t_i}$, by induction assumption $s_{t_{i}} \xrightarrow{+} s_{t_j}$, we have $s_p(t_i')  \xrightarrow{+} s_{t_j}$ in $e'$. Now that in both cases we proved $s_p(t_i)  \xrightarrow{+} s_{t_j}$ in $e'$,  therefore $s_p(t_i) \rightarrow s_{t_i} \xrightarrow{*} s_{t_j}$ in $e'$. 
 					
 				\end{enumerate}
 				
 				Since $t_i' \xrightarrow{se'} t_j$, we have $t_i' \neq t_j$, therefore $s_{t_i'} \neq s_{t_j} \Rightarrow s_{t_i'} \xrightarrow{+} s_{t_j}$. 
 				
 			\end{description}
 			
 			Combining base case and induction step, we can conclude that given any $t_j$ s.t. $\mathcal{W}_{t_j} \neq \emptyset$,  read-only transaction $t_i$ that $t_i \xrightarrow{se'} t_j$, we proved $s_{t_i} \xrightarrow{+}  s_{t_j}$.
 			
 		\end{enumerate}
 		
 		To conclude Step 1, given any $t_j$ s.t. $\mathcal{W}_{t_j} \neq \emptyset$,  any transaction $t_i$ that $t_i \xrightarrow{se'} t_j$, $s_{t_i} \xrightarrow{+}  s_{t_j}$.
 		
 		\item[Step 2] %$t_j$ is a read-only transaction, i.e. $\mathcal{W}_{t_j} = \emptyset$:
 		
 		%Therefore $s_p(t_j) =\max\{\max_{o_j \in \Sigma_{t_j}}\{ \sfomath{o_j} \},s_{t_{j-1}} \} $, where $t_{j-1}$ denotes the transaction precede $t_j$ in session $se'$.
 		
 		Now we want to prove that in $e'$, $\forall t_i \xrightarrow{se'} t_j: s_{t_i} \xrightarrow{+} s_{t_j}$. 
 		
 		First we prove that for any $t_{i-1}, t_i \in \mathcal{T}_{se'}$, where $t_{i-1}$ denotes the transaction that directly precede $t_i$ in session $se'$, we have $s_{t_{i-1}} \xrightarrow{+} s_{t_{i}}$.
 		
 		If $\mathcal{W}_{{t_i}} \neq \emptyset$, from the conclusion of Step 1, we have $s_{t_{i-1}} \xrightarrow{+} s_{t_{i}}$. 
 		
 		If ${t_i}$ is a read-only transaction, $s_p(t_i) =\max\{\max_{o_i \in \Sigma_{t_i}}\{ \sfomath{o_i} \},s_{t_{i-1}} \} $.  Since  $ \max\{\max_{o_i \in \Sigma_{t_i}}\{ \sfomath{o_i} \},s_{t_{i-1}} \} \geq s_{t_{i-1}}$, we have $s_{t_{i-1}} \xrightarrow{*}  s_p(t_i) $, therefore $s_{t_{i-1}} \xrightarrow{+} s_{t_i}$.
 		
 		Therefore, consider $t_1 \xrightarrow{se'} t_2 \xrightarrow{se'} \dots \xrightarrow{se'} t_{k} $, that $\mathcal{T}_{se'} = \{t_1,\dots,t_k\}$, we have $s_{t_1} \xrightarrow{+} s_{t_2} \xrightarrow{+} \dots \xrightarrow{+} s_{t_k}$. Therefore we proved that $\forall t_i \xrightarrow{se'} t_j: s_{t_i} \xrightarrow{+} s_{t_j}$. 
 		
 	\end{description}
 	
 	\begin{table}
 		\footnotesize{
 			\begin{center}
 				\begin{tabular}{|c|c|}
 					\hline
 					Read-My-Writes (RMW)& $\prereadmath{e}{\mathcal{T}_{se}} \wedge \forall o \in \Sigma_t: \forall t'\xrightarrow{se} t:\mathcal{W}_{t'} \neq \emptyset \Rightarrow s_{t'} \xrightarrow{*}sl_o$\\ 
 					\hline
 					Monotonic Reads (MR) & $\prereadmath{e}{\mathcal{T}_{se}} \wedge \ircmath{e}{t} \wedge \forall o \in \Sigma_t: \forall t'\xrightarrow{se}t: \forall o' \in \Sigma_{t'}: sf_{o'}\xrightarrow{*}sl_o $\\
 					\hline
 					Monotonic Writes (MW) & $\prereadmath{e}{\mathcal{T}_{se}} \wedge \forall se' \in SE: \forall t_i \xrightarrow{se'} t_j: (\mathcal{W}_{t_i} \neq \emptyset \wedge
 					\mathcal{W}_{t_j} \neq \emptyset) \Rightarrow s_{t_i} \xrightarrow{+} s_{t_j} $\\
 					\hline
 					Writes-Follow-Reads (WFR) & $\prereadmath{e}{\mathcal{T}} \wedge \forall se' \in SE: \forall t_i\xrightarrow{se'}t_j: \forall o_i \in \Sigma_{t_i}:\mathcal{W}_{t_j} \neq \emptyset \Rightarrow sf_{o_i} \xrightarrow{+} s_{t_j} $\\
 					\hline
 					Causal Consistency (CC) &  \tabincell{c}{$ \prereadmath{e}{\mathcal{T}} \wedge \ircmath{e}{t} \wedge (\forall o \in \Sigma_t: \forall t' \xrightarrow{se} t:  s_{t'} \xrightarrow{*} sl_o) $\\ $\wedge (\forall se' \in SE: \forall t_i \xrightarrow{se'} t_j: s_{t_i} \xrightarrow{+} s_{t_j})$ } \\
 					\hline

 				\end{tabular}
 			\end{center}
 		}
 		\caption{Session Guarantees}
 		
 	\end{table}
 	
 	
 	Therefore we proved that in $e'$, $\forall se' \in SE: \forall t_i \xrightarrow{se'} t_j: s_{t_i} \xrightarrow{+} s_{t_j} $.
 	
 	 	\begin{clm}
 	 		$\forall t \in T_{se} :\sessionmath{RMW}{se}{t}{e'}  \wedge \sessionmath{MR}{se}{t}{e'} $.
 	 		\yp{The reason for splitting the proofs for session is because I need the conclusion above to prove RMW and MR}
 	 		\label{claim:RMWMR}
 	 	\end{clm}
 	\begin{proof}
 		 		
 		 		Since we have $\forall t \in T_{se} :\sessionmath{RMW}{se}{t}{e}  \wedge \sessionmath{MR}{se}{t}{e} $, now we consider $e'$.
 		
 			\begin{description}
 				\item[RMW] 
 				 Consider $\forall o \in \Sigma_t: \forall t'\xrightarrow{se} t:\mathcal{W}_{t'} \neq \emptyset$
 					\begin{description}
 						\item[$o = r(k,v)$] Since $\mathcal{RS}_{e'}(o) = \{s \in \mathcal{S}_e | 
 						s \xrightarrow{*} s_p \wedge\big ( (k,v) \in s \vee (\exists w(k,v) \in \Sigma_t: w(k,v) \xrightarrow{to} r(k,v)) \big)\}$, and $\slomath{o}$ is the last state in $\mathcal{RS}_{e'}(o)$, therefore either $\slomath{o} = s_p(t)$, or $\slomath{o} = s_p(\hat{t})$, where $\hat{t}$ is the first transaction that change the value of $k$ to $v'\neq v$, therefore $k \in \mathcal{W}_{\hat{t}}$, i.e. $\mathcal{W}_{\hat{t}} \neq \emptyset$. 
 						\begin{enumerate}
 							\item $\slomath{o} = s_p(t)$: Since we have proved that $e'$, $\forall se' \in SE: \forall t_i \xrightarrow{se'} t_j: s_{t_i} \xrightarrow{+} s_{t_j} $, and we know that $t' \xrightarrow{se} t$, therefore $s_{t'} \xrightarrow{+} s_{t}$. Therefore we have $s_{t'} \xrightarrow{*} s_p(t)$, hence we have $s_{t'} \xrightarrow{*} \slomath{o}$.
 							
 							\item $\slomath{o} = s_p(\hat{t})$: Since $e$ satisfies $\forall t \in T_{se} :\sessionmath{RMW}{se}{t}{e} $, i.e. $s_{t'} \xrightarrow{*} \slomath{o}$ in $e$. Since $\hat{t}$ changed the value of the key $o$ reads, therefore $\slomath{o} \xrightarrow{+} s_{\hat{t}}$ in $e$. Combine $s_{t'} \xrightarrow{*} \slomath{o}$ and $\slomath{o} \xrightarrow{+} s_{\hat{t}}$, we have $s_{t'} \xrightarrow{+} s_{\hat{t}}$ in $e$. Since $\mathcal{W}_{t'} \neq \emptyset \wedge \mathcal{W}_{\hat{t}} \neq \emptyset$,  they are applied in $e'$ in the same order as in $e$, therefore we have $s_{t'} \xrightarrow{+} s_{\hat{t}}$ in $e'$. Therefore we have $s_{t'} \xrightarrow{*} s_p(\hat{t})$, hence we have $s_{t'} \xrightarrow{*} \slomath{o}$.
 						\end{enumerate}
 						
 						\item[$o=w(k,v)$] Since we have proved that $e'$, $\forall se' \in SE: \forall t_i \xrightarrow{se'} t_j: s_{t_i} \xrightarrow{} s_{t_j} $, and we know that $t' \xrightarrow{se} t$, therefore $s_{t'} \xrightarrow{+} s_{t}$. Therefore we have $s_{t'} \xrightarrow{*} s_p(t)$, hence we have $s_{t'} \xrightarrow{*} \slomath{o}$.
 					\end{description} 
 					
 				Therefore we have proved that $\forall o \in \Sigma_t: \forall t'\xrightarrow{se} t:\mathcal{W}_{t'} \neq \emptyset \Rightarrow s_{t'} \xrightarrow{*}sl_o$.
 				
 				By Claim~\ref{claim:pretrue}, $\prereadmath{e'}{\mathcal{T}}$ is true and $\mathcal{T}_{se} \subseteq \mathcal{T}$, by Lemma~\ref{prereadlemma}, we have $\prereadmath{e'}{\mathcal{T}_{se}}$ is true. Therefore we have proved that  $\prereadmath{e'}{\mathcal{T}_{se}} \wedge \forall o \in \Sigma_t: \forall t'\xrightarrow{se} t:\mathcal{W}_{t'} \neq \emptyset \Rightarrow s_{t'} \xrightarrow{*}sl_o$, i.e. $\forall t \in T_{se} :\sessionmath{RMW}{se}{t}{e'}$.
 				
 				
 				\item[MR] 
 	
 				
 				First we prove that $\forall o \in \Sigma_t: \forall t'\xrightarrow{se}t: \forall o' \in \Sigma_{t'}: sf_{o'}\xrightarrow{*}sl_o $:
 				\begin{description}
 					\item[$o' = r(k,v)$]
 					
 					If $\sfomath{o'}$ exists, then it must created by applying an update transaction $\hat{t'} \in \mathcal{T}$ which updates key $k$ with value $v$, i.e. $\sfomath{o'} = s_{\hat{t'}}$, $k \in \mathcal{W}_{\hat{t'}}$ (note that $\mathcal{W}_{\hat{t'}} \neq \emptyset$).
 					
 					 \begin{description}
 					 	\item[$o = r(k,v)$] Since $\mathcal{RS}_{e'}(o) = \{s \in \mathcal{S}_e | 
 					 s \xrightarrow{*} s_p \wedge\big ( (k,v) \in s \vee (\exists w(k,v) \in \Sigma_t: w(k,v) \xrightarrow{to} r(k,v)) \big)\}$, and $\slomath{o}$ is the last state in $\mathcal{RS}_{e'}(o)$, therefore either $\slomath{o} = s_p(t)$, or $\slomath{o} = s_p(\hat{t})$, where $\hat{t}$ is the first transaction that change the value of $k$ to $v'\neq v$, therefore $k \in \mathcal{W}_{\hat{t}}$, i.e. $\mathcal{W}_{\hat{t}} \neq \emptyset$. 
 					
 						\begin{enumerate}
 							\item $\slomath{o} = s_p(t)$: Since we have proved that $e'$, $\forall se' \in SE: \forall t_i \xrightarrow{se'} t_j: s_{t_i} \xrightarrow{+} s_{t_j} $, and we know that $t' \xrightarrow{se} t$, therefore $s_{t'} \xrightarrow{+} s_{t}$ in $e'$. Therefore we have $s_{t'} \xrightarrow{*} s_p(t)$ in $e'$, hence we have $s_{t'} \xrightarrow{*} \slomath{o}$ in $e'$. Since $\prereadmath{e'}{\mathcal{T}_{se}}$, by lemma \ref{sfolemma}, we have $\sfomath{o'} \xrightarrow{*} s_{t'}$ in $e'$, therefore $\sfomath{o'} \xrightarrow{*} \slomath{o}$ in $e'$. 
 							
 							\item $\slomath{o} = s_p(\hat{t})$: Since $e$ satisfies $\forall t \in T_{se} :\sessionmath{MR}{se}{t}{e} $, i.e. $\sfomath{o'} \xrightarrow{*} \slomath{o}$ in $e$. Since $\hat{t}$ changed the value of the key $o$ reads, therefore $\slomath{o} \xrightarrow{+} s_{\hat{t}}$ in $e$. Combine $\sfomath{o'} \xrightarrow{*} \slomath{o}$ and $\slomath{o} \xrightarrow{+} s_{\hat{t}}$, we have $\sfomath{o'} \xrightarrow{+} s_{\hat{t}}$ in $e$. Note that we have argued that $\sfomath{o'} = s_{\hat{t'}}$ and both ${\hat{t'}} $ and $\hat{t}$ are update transactions, therefore they are applied in $e'$ in the same order as in $e$, therefore we have $\sfomath{o'} \xrightarrow{+} s_{\hat{t}}$ in $e'$. Therefore we have $\sfomath{o'} \xrightarrow{*} s_p(\hat{t})$ in $e'$, hence we have $\sfomath{o'} \xrightarrow{*} \slomath{o}$ in $e'$.
 						\end{enumerate}
 							\item[$o=w(k,v)$] Since $\mathcal{RS}_{e'}(o) = \{s \in \mathcal{S}_e | 
 							s \xrightarrow{*} s_p\}$, therefore $\slomath{o} = s_p(t)$. Since we have proved that $e'$, $\forall se' \in SE: \forall t_i \xrightarrow{se'} t_j: s_{t_i} \xrightarrow{} s_{t_j} $, and we know that $t' \xrightarrow{se} t$, therefore $s_{t'} \xrightarrow{+} s_{t}$. Therefore we have $s_{t'} \xrightarrow{*} s_p(t)$, hence we have $s_{t'} \xrightarrow{*} \slomath{o}$. Since $\prereadmath{e'}{\mathcal{T}_{se}}$, by lemma \ref{sfolemma}, we have $\sfomath{o'} \xrightarrow{+} s_{t'}$ in $e'$, therefore $\sfomath{o'} \xrightarrow{+} \slomath{o}$ in $e'$. 
 						\end{description} 
 					
 					\item[$o'=w(k,v)$] Since for write operations, $\sfomath{o'} = s_0$, $\sfomath{o'} \xrightarrow{*} \slomath{o}$ trivially holds.
 				\end{description} 
 				
 				
 				
 				Now we prove that $\ircmath{e'}{t}$, i.e. 
 				$\forall o, \, o' \in \Sigma_t:
 				o'\xrightarrow{to} o \Rightarrow s\hspace{-0.1em}f_{o'} \xrightarrow{*}sl_o$
 				\begin{description}
 					\item[$o' = r(k,v)$]
 					
 					If $\sfomath{o'}$ exists, then it must created by applying an update transaction $\hat{t'} \in \mathcal{T}$ which updates key $k$ with value $v$, i.e. $\sfomath{o'} = s_{\hat{t'}}$, $k \in \mathcal{W}_{\hat{t'}}$ (note that $\mathcal{W}_{\hat{t'}} \neq \emptyset$).
 					
 					\begin{description}
 						\item[$o = r(k,v)$] Since $\mathcal{RS}_{e'}(o) = \{s \in \mathcal{S}_e | 
 						s \xrightarrow{*} s_p \wedge\big ( (k,v) \in s \vee (\exists w(k,v) \in \Sigma_t: w(k,v) \xrightarrow{to} r(k,v)) \big)\}$, and $\slomath{o}$ is the last state in $\mathcal{RS}_{e'}(o)$, therefore either $\slomath{o} = s_p(t)$, or $\slomath{o} = s_p(\hat{t})$, where $\hat{t}$ is the first transaction that change the value of $k$ to $v'\neq v$, therefore $k \in \mathcal{W}_{\hat{t}}$, i.e. $\mathcal{W}_{\hat{t}} \neq \emptyset$. 
 						
 						\begin{enumerate}
 							\item $\slomath{o} = s_p(t)$: Since we showed $\prereadmath{e'}{\mathcal{T}}$ is true in Claim~\ref{claim:pretrue} and $o' \in \Sigma_{t}$, by lemma \ref{sfolemma}, we have $\sfomath{o'} \xrightarrow{+} s_{t}$ in $e'$, therefore $\sfomath{o'} \xrightarrow{*} s_p(t) $ in $e'$, i.e. $\sfomath{o'} \xrightarrow{*} \slomath{o} $ in $e'$. 
 							
 							\item $\slomath{o} = s_p(\hat{t})$: Since $e$ satisfies $\forall t \in T_{se} :\sessionmath{MR}{se}{t}{e} $, i.e. $\sfomath{o'} \xrightarrow{*} \slomath{o}$ in $e$. Since $\hat{t}$ changed the value of the key $o$ reads, therefore $\slomath{o} \xrightarrow{+} s_{\hat{t}}$ in $e$. Combine $\sfomath{o'} \xrightarrow{*} \slomath{o}$ and $\slomath{o} \xrightarrow{+} s_{\hat{t}}$, we have $\sfomath{o'} \xrightarrow{+} s_{\hat{t}}$ in $e$. Note that we have argued that $\sfomath{o'} = s_{\hat{t'}}$ and both ${\hat{t'}} $ and $\hat{t}$ are update transactions, therefore they are applied in $e'$ in the same order as in $e$, therefore we have $\sfomath{o'} \xrightarrow{+} s_{\hat{t}}$ in $e'$. Therefore we have $\sfomath{o'} \xrightarrow{*} s_p(\hat{t})$ in $e'$, hence we have $\sfomath{o'} \xrightarrow{*} \slomath{o}$ in $e'$.
 						\end{enumerate}
 						\item[$o=w(k,v)$] Since $\mathcal{RS}_{e'}(o) = \{s \in \mathcal{S}_e | 
 						s \xrightarrow{*} s_p\}$, therefore $\slomath{o} = s_p(t)$. Since we showed $\prereadmath{e'}{\mathcal{T}}$ is true in Claim~\ref{claim:pretrue} and $o' \in \Sigma_{t}$, by lemma \ref{sfolemma}, we have $\sfomath{o'} \xrightarrow{+} s_{t}$ in $e'$, therefore $\sfomath{o'} \xrightarrow{*} s_p(t) $ in $e'$, i.e. $\sfomath{o'} \xrightarrow{*} \slomath{o} $ in $e'$. 
 					\end{description} 
 					
 					\item[$o'=w(k,v)$] Since for write operations, $\sfomath{o'} = s_0$, $\sfomath{o'} \xrightarrow{*} \slomath{o}$ trivially holds.
 				\end{description} 
 				
 				Therefore we have proved that $\ircmath{e'}{t} \wedge \forall o \in \Sigma_t: \forall t'\xrightarrow{se}t: \forall o' \in \Sigma_{t'}: sf_{o'}\xrightarrow{*}sl_o $.
 				
 				By Claim~\ref{claim:pretrue}, $\prereadmath{e'}{\mathcal{T}}$ is true and $\mathcal{T}_{se} \subseteq \mathcal{T}$, by Lemma~\ref{prereadlemma}, we have $\prereadmath{e'}{\mathcal{T}_{se}}$ is true. Therefore we have proved that  $\prereadmath{e'}{\mathcal{T}_{se}} \wedge \ircmath{e'}{t} \wedge \forall o \in \Sigma_t: \forall t'\xrightarrow{se}t: \forall o' \in \Sigma_{t'}: sf_{o'}\xrightarrow{*}sl_o $, i.e. $\forall t \in T_{se} :\sessionmath{MR}{se}{t}{e'}$.
 			\end{description}
 	\end{proof}
 	
 
 	
 	Now we prove that the $e'$ also satisfy $\forall t \in T_{se} :\sessionmath{CC}{se}{t}{e'} $.
 	
 	By Claim~\ref{claim:pretrue}, $\prereadmath{e'}{\mathcal{T}}$ holds.
	
	By Claim~\ref{claim:RMWMR}, $\forall t \in T_{se} :\sessionmath{MR}{se}{t}{e'}$, therefore $\ircmath{e'}{t}$ holds. 
	
	We have proved that in $e'$, $\forall se' \in SE: \forall t_i \xrightarrow{se'} t_j: s_{t_i} \xrightarrow{+} s_{t_j} $.
	
	Now we want to prove that $\forall t \in T_{se} : (\forall o \in \Sigma_t: \forall t' \xrightarrow{se} t:  s_{t'} \xrightarrow{*} sl_o) $. 
	
	By Claim~\ref{claim:RMWMR}, $\forall t \in T_{se} :\sessionmath{RMW}{se}{t}{e'}$, therefore  $\forall t \in T_{se} : (\forall o \in \Sigma_t: \forall t' \xrightarrow{se} t:  \mathcal{W}_{t'} \neq \emptyset \Rightarrow s_{t'} \xrightarrow{*} sl_o)$ holds. 
	
	Now we want to prove that given any transaction $t\in T_{se}$, $\forall o \in \Sigma_t: \forall t' \xrightarrow{se} t, \mathcal{W}_{t'} =\emptyset \Rightarrow s_{t'} \xrightarrow{*}\slomath{o}$ by induction .

	
	\begin{description}
		
		\item[Base case] Consider the first read-only transaction $t'$ in session $se$, remember that we choose the parent state of a read-only transaction as $s_p(t') = \max\{\max_{o' \in \Sigma_{t'}}\{\sfomath{o'}\}, s_{t'_{-1}}\}$, where $ t'_{-1}$ denotes the transaction that directly precedes $t'$ in session $se$.  Therefore either $s_p(t') = \max_{o' \in \Sigma_{t'}}\{ \sfomath{o'} \} $ or $s_p({t'}) = s_{t'_{-1}} \wedge \mathcal{W}_{t'_{-1}} \neq \emptyset$.
		
			\begin{enumerate}
				\item 
					If $s_p(t') = \max_{o' \in \Sigma_{t'}}\{ \sfomath{o'} \} $: By Claim~\ref{claim:RMWMR}, $\forall t \in T_{se} :\sessionmath{MR}{se}{t}{e'}$, we have $\forall o' \in \Sigma_{t'}: \sfomath{o'} \xrightarrow{*} \slomath{o}$, therefore $\max_{o' \in \Sigma_{t'}} \{\sfomath{o'} \} \xrightarrow{*} \slomath{o}$ in $e'$. Now we have $s_p({t'}) \xrightarrow{*} \slomath{o}$ in $e'$.
				
				\item
					If $s_p({t'}) = s_{t'_{-1}} \wedge \mathcal{W}_{t'_{-1}} \neq \emptyset$: Consider $(t'_{-1}, t)$, since we know that $t'_{-1} \xrightarrow{se} t' \xrightarrow{se} t $, we have $ t'_{-1} \xrightarrow{se} t$. Given that $\mathcal{W}_{t'_{-1}} \neq \emptyset$, therefore by Claim~\ref{claim:RMWMR}, $\forall t \in T_{se} :\sessionmath{RMW}{se}{t}{e'}$, we have $s_{t'_{-1}} \xrightarrow{*} \slomath{o}$ in $e'$. Again we have $s_p({t'}) \xrightarrow{*} \slomath{o}$ in $e'$.
				
			\end{enumerate}

		
		Now we argue that $s_p(t') \neq \slomath{o}$: since $t'$ is a read-only transaction, $\forall (k,v) \in s_p(t')  \Rightarrow (k,v) \in s_{t'}$. Since we have proved that in $e'$, $\forall se' \in SE: \forall t_i \xrightarrow{se'} t_j: s_{t_i} \xrightarrow{+} s_{t_j} $, therefore we have $s_{t'} \xrightarrow{+} s_{t}$. Therefore $s_p(t') \in \mathcal{RS}_{e'}(o) \Rightarrow s_{t'} \in \mathcal{RS}_{e'}(o)$, i.e. $s_p(t') \neq \slomath{o}$.
		
		Therefore we have $s_p({t'}) \xrightarrow{+} \slomath{o}$, i.e. $s_p({t'}) \rightarrow s_{t'}\xrightarrow{*} \slomath{o}$.
		
		
		\item[Induction step] Assume that the k-th read-only transaction $t'$ in $se$, s.t. $t' \xrightarrow{se} t$, satisfies $\forall o \in \Sigma_t: s_{t'} \xrightarrow{*}\slomath{o}$. Now we we consider the (k+1)-th read-only transaction $t''$ in $se$, s.t. $t'' \xrightarrow{se} t$. Note that either $t'$ directly precedes $t''$ in $se$, or there exists an update transaction that directly precedes $t''$ in $se$.
		
		Again either $s_p(t'') = \max_{o'' \in \Sigma_{t''}}\{ \sfomath{o''} \} $ or $s_p({t''}) = s_{t''_{-1}}$, where $ t''_{-1}$ denotes the transaction that directly precedes $t''$ in session $se$. Note that either $\mathcal{W}_{t''_{-1}}= \emptyset \Rightarrow t''_{-1} = t'$ or $\mathcal{W}_{t''_{-1}} \neq \emptyset$.
		
			\begin{enumerate}
				\item 
				If $s_p(t'') = \max_{o'' \in \Sigma_{t''}}\{ \sfomath{o''} \} $: By Claim~\ref{claim:RMWMR}, $\forall t \in T_{se} :\sessionmath{MR}{se}{t}{e'}$, we have $\forall o'' \in \Sigma_{t''}: \sfomath{o''} \xrightarrow{*} \slomath{o}$, therefore $\max_{o'' \in \Sigma_{t'}} \{\sfomath{o''} \} \xrightarrow{*} \slomath{o}$ in $e'$. Now we have $s_p({t''}) \xrightarrow{*} \slomath{o}$ in $e'$.
			
				\item
				If $s_p({t''}) = s_{t''_{-1}} $: 
				If $\mathcal{W}_{t''_{-1}}= \emptyset$, i.e. $ t''_{-1} = t'$, by induction assumption  $s_{t''_{-1}}  = s_{t'} \xrightarrow{*}  \slomath{o}$, i.e. $s_p(t'') \xrightarrow{*} \slomath{o}$.
				If $\mathcal{W}_{t'_{-1}} \neq \emptyset$, consider $(t''_{-1}, t)$, since we know that $t''_{-1} \xrightarrow{se} t'' \xrightarrow{se} t $, we have $ t''_{-1} \xrightarrow{se} t$, therefore by Claim~\ref{claim:RMWMR}, $\forall t \in T_{se} :\sessionmath{RMW}{se}{t}{e'}$, we have $s_{t''_{-1}} \xrightarrow{*} \slomath{o}$ in $e'$. 
				Again we have $s_p({t''}) \xrightarrow{*} \slomath{o}$ in $e'$.
				
				
			\end{enumerate}
		
		
		
	Now we argue that $s_p(t'') \neq \slomath{o}$: since $t''$ is a read-only transaction, $\forall (k,v) \in s_p(t'')  \Rightarrow (k,v) \in s_{t''}$. Since we have proved that in $e'$, $\forall se' \in SE: \forall t_i \xrightarrow{se'} t_j: s_{t_i} \xrightarrow{+} s_{t_j} $, therefore we have $s_{t''} \xrightarrow{+} s_{t}$. Therefore $s_p(t'') \in \mathcal{RS}_{e'}(o) \Rightarrow s_{t''} \in \mathcal{RS}_{e'}(o)$, i.e. $s_p(t'') \neq \slomath{o}$.
	
	Therefore we have $s_p({t''}) \xrightarrow{+} \slomath{o}$, i.e. $s_p({t''}) \rightarrow s_{t''}\xrightarrow{*} \slomath{o}$.
		
		Therefore we proved that $s_{t''} \xrightarrow{*} \slomath{o}$. 
		
	\end{description}
	
	Combining base case and induction step, we can conclude that $\forall t\in T_{se}$, $\forall o \in \Sigma_t: \forall t' \xrightarrow{se} t, \mathcal{W}_{t'} =\emptyset \Rightarrow s_{t'} \xrightarrow{*}\slomath{o}$.
	
	Therefore, we proved that $\forall t \in T_{se} : (\forall o \in \Sigma_t: \forall t' \xrightarrow{se} t:  s_{t'} \xrightarrow{*} sl_o) $. 
	
	Therefore, we proved that $ \prereadmath{e}{\mathcal{T}} \wedge \ircmath{e}{t} \wedge (\forall o \in \Sigma_t: \forall t' \xrightarrow{se} t:  s_{t'} \xrightarrow{*} sl_o)  \wedge (\forall se' \in SE: \forall t_i \xrightarrow{se'} t_j: s_{t_i} \xrightarrow{+} s_{t_j})$, i.e. $\forall t \in T_{se} :\sessionmath{CC}{se}{t}{e'}$.
	
\end{proof}



==> problem-current2.tex <==
\section{Abstracting guarantees from implementation}
\label{s:problemcurrent}

\nc{Don't Like the title}

* Modern applications process and store large amounts of data in geographically distinct locations.
During so reliably and at scale is challenging.
\nc{ISSUE: not talking about data processing systems here, only databases/storage systems}
* As a result, applications offload the task of storing the data to storage systems:
these systems should ensure data is stored durably, accessed efficiently, at high scale
and across failures without concerning the application with how this is achieved.
* This concern is evident in the architecture of these systems: most expose
a simple front-end to applications that hides the highly complex protocols that
ensure data can stored reliably and delivered at high performance.
* Consider for example Cassandra ~\cite{Chihoub2012}, a peer-to-peer large-scale distributed
storage system: all client requests access a {\em coordinator}
node. That node is then responsible for routing the client request  to the appropriate
storage node based on the existing cluster configuration. The application itself does not
have to worry about node churn, data transfer, or cluster configuration.
* Likewise, the MySQL Cluster exposes a number of front-end to applications.
Durability is then achieved under the hood, via synchronous master-slave replication,
while scalability is achieved by sharding data and adding more nodes online. The front-end is then, like
in Cassandra, responsible for routing the client request to the appropriate node
in the system.
\nc{ISSUE: there's some work in how the application can shard the data manually to
achieve better performance. Does that break the abstraction?}
\nc{ISSUE2: I'm intentionally omitting any mention of consistency here}
* Cloud-based storage systems like Azure Storage and S3 have proven popular for
similar reasons: the application obtains strong performance and durability guarantees
without worrying about how these are achieved.

* This separation of concern, however, breaks down when considering the guarantees
provided by these systems on the properties of the data itself. Guarantees on data can be divided
into two: coherence and consistency~\cite{}. \nc {i'm going to not mention isolation
here and argue that isolation is a way to achieve consistency?}.
* Data coherence~\cite{} defines the relationship between different copies of data, located on
different replicas. This is akin to the notion of cache coherence. * Data consistency
on the other hand constrains the relationship between concurrent data accesses.
This is akin to the notion of consistency in weak memory systems~\cite{}.
\nc{this is the most natural way  i found to define what i mean by
  ``properties of the data''. The downside of this approach is that i never talk
about coherence and consistency again. I'm also explicitly not mentioning
the notion of consistency in distributed systems or databases. Good idea? }
* Current systems do not provide clean guarantees on coherence and consistency
that are independent of their implementation.
* One hand, certain guarantees can only be understood with respect to their specific 
implementation.
\nc{i don't think all the examples should be there, i'm giving a list
so that we can pick the most compelling one/two/three}.
* Consider for example the notion of quorum consistency in Cassandra:
a write will return once it has been written to a quorum of replicas. Likewise, a read
will return the most recent value obtained from a quorum.
An application must now be aware that the system is an asynchronously replicated
system.
\nc{i don't think this is a good example. it's pretty intuitive and the only
implementation detail I need to know is replicated/not replicated}.
* Similarly, consider the definition of snapshot isolation~\cite{Fekete2005,Berenson,Science1999a}:
snapshot isolation \nc{is that technically based on specific implementation? first updater wins and first
committer wins seem fairly low level to me}: the definition of this isolation level
relies on three properties: 1) snapshot reads, where transactions should read
the most recent snapshot of the system 2) a centralised counter that assigns monotonically
increasing timestamps 3) the first-committer or first-updater-wins rules.
* Similarly, the definition of parallel snapshot isolation~\cite{Sovran2011b},
an isolation model defined to remove the bottleneck associated with the centralised counter
in snapshot isolation was defined exclusively in terms of a specific system: Walter~\cite{Sovran2011b},
and assumed, for example, causally consistent replication across sites, and
``primary sites'' to enforce the first committer rule.
\nc{i think this is a nicer example. The downside is that this an academic
system, not an industrial one. I also need to be careful about being
fair to Alexey's work. He has defined PSI in an independent fashion
though his model makes some pretty strong assumptions}.
* Reddis: Reddis implements linearizable multi-write transactions within
the same partition only. This forces the programmer to think about data
partitioning in order to know that writes will be execute atomically.
* As above, Azure Storage ensures that writes within the same partitions
will be executed atomically, but writes across partitions may not.
* Recently, Attiya et al.\cite{Attiya} defined observal causal consistency
as the strongest consistency level that guarantees high availability.
However, their model makes strong assumptions about the communication
model of their idealised data-store: namely, that a replica must never
contact another server before responding to a request.
Their model is, as a result, unapplicable to many modern datastores that
provide a mixture of guarantees, like Cassandra:
Cassadra's QUORUM operation replicates an operation synchronously to a quorum of replicas, 
and asynchronously to the remaining members of the cluster

* On the other, what is nominally the same guarantee can actually lead to different
results~\nc{reformulate ... a guarantee does not lead to results} based on the
implementation.
* Consider the definition of serializability, 
Phil Bernstein's intiialy definition of serializability 
ignores the ability of the storage to re-order writes.
The following execution is thus not serializable in his definition
$(R_1(X1)W_2(X2)W_1(X3))$ but serializable under the definition of Atul, which
does allow for write re-ordering. Similarly, in MySQL, the following execution
is allowed if and only if X is not a primary key $S_1 RSCAN_1(Table T) W_2(T,X) C_1 C_2$.
This is due to their implementation of indices where writes lock the index only.
\nc{not ideally phrased + ISSUE: our current model does not consider scans. I don't think this would
be too hard based on, but it just makes thing look less clean}

* Separating data consistency from implementation has proven
to be challenging  due to the diversity of the current
eco-systems. \nc{neeed for larger scale data processing. develop storage systems to hadnle taht. no
time to think properly. But realised that sacrifified programmability and portability. Push back now?
explicity designed for a set of applications, and developers. But then the set of applications expand
}

They differ along three main axis:
\begin{itemize}
\item they differ in terms of the guarantees provided: MySQL Cluster guarantees applications
read-committed ; Spanner and Voldemort guarantee serializability, Pileus (and its
commercial cousin DocumentDB) session guarantees, while Cassandra provides a
restrictive form of transactions. \la{they don't have get it right just once, 
but they have to het right for a large nb of guarantees, and conversely
the same guarantee has to be provided over many different implementations.
} \nc{say why they got it wrong. race to arms.}
\item independently of the guarantees provided, their implementation varies
significantly: PostgresSQL is a fully multi-versioned system,
MySQL Cluster is 2-versioned, and \nc{Insert a single versioned system}. All
store data on disk, while Microsoft SQL Cluster's Hekaton, optimises its design
for memory-based tables. Similarly, MySQL Cluster relies on
locks for concurrency control, while PostgresSQL relies on a snapshot based
concurrency control mechanism, and Hekaton relies on an optimistic concurrency
control protocol.
\item finally, the replication strategy of these systems also differ: some,
like Pileus, rely on a single master with asynchronous propagation of updates,
others opt for synchronous multi-master replication~\cite{}, while some,
like Dynamo~\cite{} choose asynchronous multi-master replication. Many
provide a mixture of these guarantees: Cassadra's QUORUM operation
replicates an operation synchronously to a quorum of replicas, and asynchronously
to the remaining members of the cluster.
\end{itemize}

To achieve the idealised goal of separating guarantees on data from
implementation, we believe that consistency models should be defined
exclusively from the application perspective, at the granularity of what
the application can observe - namely, atomic state transitions. 

Specifically, the model should
\begin{enumerate}
\item should be oblivious to whether the system is replicated
\item should be oblivious to the strategy used for replication
\item should be oblivious tto the local isolation level of each site
\item should never mention something that the application itself cannot 
observe \nc{rephrase}
\end{enumerate}


==> psi.tex <==
\subsection{PSI and PL2+}

\begin{lemma}
	$\prereadmath{e}{\hat{t}} \Rightarrow \forall t \in \ddependsmath{e}{\hat{t}}, s_t \xrightarrow{+} s_{\hat{t}}$
	\label{lemma:preddirect}
\end{lemma}

\begin{proof}
	Consider any $t \in \ddependsmath{e}{\hat{t}}$, therefore either case, or both cases can happen:
	\begin{enumerate}
		\item $t \in 	\{t| \exists o \in \Sigma_{\hat{t}}, t=t_{{sf_o}}\},$ by $\prereadmath{e}{\hat{t}}$, we have $\forall o, \sfomath{o} \xrightarrow{+} s_{\hat{t}}$, consider the $o$, that $t = t_{\sfomath{o}}$, we have $s_t = \sfomath{o} \xrightarrow{+} s_{\hat{t}}$.
		
		\item $t \in \{t|s_{t} \xrightarrow{+} s_{\hat{t}} \wedge \mathcal{W}_{\hat{t}} \cap \mathcal{W}_{t} \neq \emptyset \}$, trivially we have $s_t \xrightarrow{+} s_{\hat{t}}$.
	\end{enumerate}
\end{proof}

\begin{lemma}
	$\prereadmath{e}{\mathcal{T}} \Rightarrow \forall t' \in \dependsmath{e}{t}: s_{t'} \xrightarrow{+} s_t$.
	\label{lemma:predtrans}
\end{lemma}

\begin{proof}
	\begin{description}
		\item[Base case] Consider the first applied transaction $t_1$, we want to prove that $\forall t$, s.t. $s_t \xrightarrow{*} s_{t_1} : \forall t' \in \dependsmath{e}{t}: s_{t'} \xrightarrow{*} s_{t}$. 
		
		Consider any $t \in \ddependsmath{e}{t_1}$, by Lemma~\ref{lemma:preddirect}, we have $s_t \xrightarrow{+} s_{t_1}$. 
		Since $t_1$ is the first applied transaction, there does not exist a $t \neq t_1$ that $s_{t} \xrightarrow{+}s_{t_1} $, therefore $\ddependsmath{e}{t_1} = \emptyset$. Therefore $\dependsmath{e}{t_1} = \emptyset$.
		Since $\dependsmath{e}{t_1} = \emptyset$, $\forall t' \in \dependsmath{e}{t_1}: s_{t'} \xrightarrow{+} s_{t_1}$ trivially follows. Note that only $t_1$ is the only transaction $t$ that $s_{t} \xrightarrow{*} s_{t_1}$,  therefore $\forall t$, s.t. $s_t \xrightarrow{*} s_{t_1} : \forall t' \in \dependsmath{e}{t}: s_{t'} \xrightarrow{+} s_{t}$ is proved.
		
		
		\item[Induction step] Assume that $\forall t$, s.t. $s_t \xrightarrow{*} s_{t_i}$, $ \forall t' \in \dependsmath{e}{t}: s_{t'} \xrightarrow{+} s_t$. 
		
		Now we prove that $\forall t$, s.t. $s_t \xrightarrow{*} s_{t_{i+1}}, \forall t' \in \dependsmath{e}{t}: s_{t'} \xrightarrow{*}s_t$. Therefore we only need to prove that $ \forall t' \in \dependsmath{e}{t_{i+1}}: s_{t'} \xrightarrow{*}s_{t_{i+1}}$.
		
		Since $\dependsmath{e}{t_{i+1}} = (\bigcup_{t \in \ddependsmath{e}{t_{i+1}}} \dependsmath{e}{t} )\cup \ddependsmath{e}{t_{i+1}}$.
		
		Therefore consider any $t' \in \dependsmath{e}{t_{i+1}}$, either $t' \in \ddependsmath{e}{t_{i+1}}$, or $ \exists t$, $t' \in \dependsmath{e}{t} \wedge t \in \ddependsmath{e}{t_{i+1}}$, or both cases can happen.
		
		\begin{enumerate}
			\item If $t' \in \ddependsmath{e}{t_{i+1}}$, by Lemma~\ref{lemma:preddirect}, we have $s_{t'}  \xrightarrow{+} s_{t_{i+1}}$.
			
			\item If $ \exists t$, $t' \in \dependsmath{e}{t} \wedge t \in \ddependsmath{e}{t_{i+1}}$: Since $t  \in \ddependsmath{e}{t_{i+1}}$, by Lemma~\ref{lemma:preddirect}, we have $s_{t}  \xrightarrow{+} s_{t_{i+1}}$, i.e. $s_t \xrightarrow{*} s_{t_i}$.
			By induction assumption, we have that $\forall t'' \in \dependsmath{e}{t}: s_{t''} \xrightarrow{+} s_{t}$.
			Note that $t' \in \dependsmath{e}{t}$, therefore we have $s_{t'} \xrightarrow{+} s_{t} \xrightarrow{+}  s_{t_{i+1}}$, i.e. we proved $s_{t'}  \xrightarrow{+}  s_{t_{i+1}}$.
		\end{enumerate}
		
		
		Combine the two cases, we proved that $\forall t' \in \dependsmath{e}{t_{i+1}}: s_{t'}  \xrightarrow{+}  s_{t_{i+1}}$.
		
		
	\end{description}
	Let $t_n$ be last transaction applied in execution $e$. Therefore by base case and induction step, we proved that $\forall t$, s.t. $s_t \xrightarrow{*} s_{t_n} : \forall t' \in \dependsmath{e}{t}: s_{t'} \xrightarrow{*} s_{t}$, since $t_n$ is the last applied transaction, therefore for $\forall t$ we have $ s_t \xrightarrow{*} s_{t_n}$, therefore the conclusion is same as $\forall t: \forall t' \in \dependsmath{e}{t}: s_{t'} \xrightarrow{*} s_{t}$.
\end{proof}

\begin{lemma}
	$\prereadmath{e}{\mathcal{T}} \Rightarrow \forall t' \in \dependsmath{e}{t}: t' \xrightarrow{ww/wr}^+ t$ in $DSG(H)$.
	\label{lemma:predchain}
\end{lemma}

\begin{proof}
	\begin{description}
		\item[Base case] Consider the first applied transaction $t_1$, we want to prove that $\forall t$, s.t. $s_t \xrightarrow{*} s_{t_1} : \forall t' \in \dependsmath{e}{t}: t' \xrightarrow{ww/wr}^+ t$ in $DSG(H)$. 
		
		Consider any $t \in \ddependsmath{e}{t_1}$, by Lemma~\ref{lemma:preddirect}, we have $s_t \xrightarrow{+} s_{t_1}$. 
		Since $t_1$ is the first applied transaction, there does not exist a $t \neq t_1$ that $s_{t} \xrightarrow{+}s_{t_1} $, therefore $\ddependsmath{e}{t_1} = \emptyset$. Therefore $\dependsmath{e}{t_1} = \emptyset$.
		Since $\dependsmath{e}{t_1} = \emptyset$, $\forall t' \in \dependsmath{e}{t_1}: t' \xrightarrow{ww/wr}^+ t_1$ trivially follows. Note that only $t_1$ is the only transaction $t$ that $s_{t} \xrightarrow{*} s_{t_1}$,  therefore $\forall t$, s.t. $s_t \xrightarrow{*} s_{t_1} : \forall t' \in \dependsmath{e}{t}: t' \xrightarrow{ww/wr}^+ t$ is proved.
		
		
		\item[Induction step] Assume that $\forall t$, s.t. $s_t \xrightarrow{*} s_{t_i}$, $ \forall t' \in \dependsmath{e}{t}: t' \xrightarrow{ww/wr}^+ t$. 
		
		Now we prove that $\forall t$, s.t. $s_t \xrightarrow{*} s_{t_{i+1}}, \forall t' \in \dependsmath{e}{t}: t' \xrightarrow{ww/wr}^+ t$. Therefore we only need to prove that $ \forall t' \in \dependsmath{e}{t_{i+1}}: t' \xrightarrow{ww/wr}^+ t_{i+1}$.
		
		Since $\dependsmath{e}{t_{i+1}} = (\bigcup_{t \in \ddependsmath{e}{t_{i+1}}} \dependsmath{e}{t} )\cup \ddependsmath{e}{t_{i+1}}$.
		
		Therefore consider any $t' \in \dependsmath{e}{t_{i+1}}$, either $t' \in \ddependsmath{e}{t_{i+1}}$, or $ \exists t$, $t' \in \dependsmath{e}{t} \wedge t \in \ddependsmath{e}{t_{i+1}}$, or both cases can happen.
		
		\begin{enumerate}
			\item If $t' \in \ddependsmath{e}{t_{i+1}}$, therefore if $t' \in \{t| \exists o \in \Sigma_{t_{i+1}}, t=t_{{sf_o}}\}
			$, we have $t_{i+1}$ read-depends on $t'$, i.e. $t' \xrightarrow{wr} t$ ; if $t' \in  \{t|s_{t} \xrightarrow{+} s_{t_{i+1}} \wedge \mathcal{W}_{t_{i+1}} \cap \mathcal{W}_{t} \neq \emptyset \}$, since by Lemma~\ref{lemma:preddirect} $s_{t'} \xrightarrow{+} s_{t_{i+1}}$. Let $x$ be the key that $x \in \mathcal{W}_{t_{i+1}} \cap \mathcal{W}_{t}$, by the way we assign the version order, we will have $x_{t'} << x_{t_{i+1}}$, therefore there must be a chain of $ww$ edges between $t'$ and $t_{i+1}$ in $DSG(H)$, where all of the transactions on the chain writes a new version of key $x$, therefore we have $t' \xrightarrow{ww}^+ t_{i+1}$. Therefore in either case $t' \xrightarrow{ww/wr}^+ t_{i+1}$.
			
			\item If $ \exists t$, $t' \in \dependsmath{e}{t} \wedge t \in \ddependsmath{e}{t_{i+1}}$: By the same analysis as above, we will have $t \xrightarrow{ww/wr}^+ t_{i+1}$.
			By Lemma~\ref{lemma:preddirect}, we have $s_t \xrightarrow{+} s_{i+1}$, therefore $s_t \xrightarrow{*} s_{i}$.
			By induction assumption, we have that $\forall t'' \in \dependsmath{e}{t}:t'' \xrightarrow{ww/wr}^+ t$.
			Note that $t' \in \dependsmath{e}{t}$, therefore we have $t' \xrightarrow{ww/wr}^+ t$. And since we have $t \xrightarrow{ww/wr}^+ t_{i+1}$, we now have $t' \xrightarrow{ww/wr}^+ t \xrightarrow{ww/wr}^+ t_{i+1}$, i.e. $t' \xrightarrow{ww/wr}^+  t_{i+1}$
		\end{enumerate}
		
		
		Combine the two cases, we proved that $\forall t' \in \dependsmath{e}{t_{i+1}}: t' \xrightarrow{ww/wr}^+  t_{i+1}$
		
		
	\end{description}
	Let $t_n$ be last transaction applied in execution $e$. Therefore by base case and induction step, we proved that $\forall t$, s.t. $s_t \xrightarrow{*} s_{t_n} : \forall t' \in \dependsmath{e}{t}: t' \xrightarrow{ww/wr}^+  t$, since $t_n$ is the last applied transaction, therefore for $\forall t$ we have $ t' \xrightarrow{ww/wr}^+  t_{n}$, therefore the conclusion is same as $\forall t: \forall t' \in \dependsmath{e}{t}: t' \xrightarrow{ww/wr}^+ t$.
\end{proof}


\[
\ddependsmath{e}{\hat{t}}=
\{t| \exists o \in \Sigma_{\hat{t}}, t=t_{{sf_o}}\}
\cup \{t|s_{t} \xrightarrow{*} s_{\hat{t}} \wedge \mathcal{W}_{\hat{t}} \cap \mathcal{W}_{t} \neq \emptyset \}\]
\[
\dependsmath{e}{\hat{t}} = (\bigcup_{t \in \ddependsmath{e}{\hat{t}}} \dependsmath{e}{t} )\cup \ddependsmath{e}{\hat{t}}
\]
\[
\commitmath{PSI}{t}{e} \equiv \prereadmath{e}{t} \wedge \forall o \in \Sigma_t: \forall t' \in \dependsmath{e}{t}: o.k \in \mathcal{W}_{t'} \Rightarrow s_{t'} \xrightarrow{*} sl_o
\]



\begin{theorem}
	Let $\mathcal{I}$ be PSI. Then $\exists e:\forall t \in \mathcal{T}:\commitmath{PSI}{t}{e} \equiv \lnot G1 \land \lnot G\text{-single}$ 
\end{theorem}

\begin{proof}
	($\Rightarrow$)First  we prove the direction that $\exists e:\forall t \in \mathcal{T}:\commitmath{PSI}{t}{e} \Rightarrow \lnot G1 \land \lnot G\text{-single}$.
	
	Let \textit{e} be an execution that $\forall t \in \mathcal{T}:\commitmath{PSI}{t}{e}$, and \textit{H} be a history for committed transactions
	$\mathcal{T}$.
	
	We first instantiate the version order for \textit{H}, denoted as $<<$, as follows: given an execution $e$ and an object $x$, $ x_i << x_j$ if and only if $x \in \mathcal{W}_{t_i} \cap \mathcal{W}_{t_j} \land  s_{t_{i}} \xrightarrow{*} s_{t_{j}} $. It follows that, for any two states such that $(x,x_i) \in T_m
	\wedge (x,x_j) \in T_n \Rightarrow s_{T_m} \xrightarrow{+} s_{T_n}$. 
	
	We first prove that $\forall t \in \mathcal{T}:\commitmath{PSI}{t}{e} \Rightarrow \lnot G1$:
	
	\begin{itemize}
		\item Let us assume that \textit{H} exhibits
		phenomenon $G1a$ (aborted reads). There
		must exists events $w_i(x_i), r_j(x_i)$ in
		H such that $t_i$ subsequently aborted. $\mathcal{T}$ and any corresponding execution $e$, however, consists only of committed
		transactions. Hence $\forall e: \not\exists s \in \mathcal{S}_e, s.t.\ s \in \RSmath{ r_j(x_i)}$: i.e. $\lnot \prereadmath{e}{t_j}$. There thus
		exists a transaction for which the commit test cannot be satisfied, for any e. We have a contradiction.
		\item  Let us assume that \textit{H} exhibits 
		phenomenon $G1b$ (intermediate reads). In an execution $e$, only the final writes of a transaction are applied. Hence,$\forall e: \not\exists s \in \mathcal{S}_e, s.t.\ s \in \RSmath{ r(x_{intermediate})}$, i.e. $\lnot \prereadmath{e}{t}$. There
		thus exists a transaction $t$, which for all e, will not 
		satisfy the commit test. We once again have a contradiction.
		\item Finally, let us assume that \textit{H} exhibits phenomenon $G1c$: $DSG(H)$ must contain a cycle
		of read/write dependencies. We consider each possible
		edge in the cycle in turn:
		\begin{itemize}
			\item[$T_i\xrightarrow{ww}T_j$] There must exist
			an object $x$ such that $x_i << x_j$ (version order). By construction, version in \textit{H} is consistent with the execution order \textit{e}: we have  $s_{T_i} \xrightarrow{*} s_{T_j}$.
			\item[$T_i\xrightarrow{wr}T_j$] There must exist
			a read $o=r_j(x_i) \in \Sigma_{t_j}$ such that
			$T_j$ reads version $x_i$ written by $T_i$. 
			By assumption, $\commitmath{PSI}{e}{T_j}$ holds.
			By $\prereadmath{e}{t}$ and Lemma~\ref{sfolemma}, we have $\sfomath{o} \xrightarrow{+} s_{T_j}$; 
			 and since $\sfomath{o}$ exists, $\sfomath{o} = s_{T_i} $.
		 It follows that  $s_{T_i} \xrightarrow{+} s_{T_j}$.
		\end{itemize}
		If a history $H$ displays phenomena $G1c$, there must exist a chain of transactions $t_i\rightarrow t_{i+1} \rightarrow ... \rightarrow t_{j}$ such that $i=j$.
		A corresponding cycle
		must thus exist in the execution \textit{e} $s_{t_i} \xrightarrow{*} s_{t_{i+1}} \xrightarrow{*} \dots \xrightarrow{*} s_{t_j}$. By definition however, a valid execution must be totally ordered. We once again have a contradiction.  
	\end{itemize}
	
	We now prove that $\forall t \in \mathcal{T}:\commitmath{PSI}{t}{e} \Rightarrow \lnot G\text{-single}$.
	
	Let us assume that \textit{H} exhibits
	phenomenon $G\text{-single}$: $DSG(H)$ must contain a directed cycle with exactly one anti-dependency edge. Let $t_1 \xrightarrow{ww/wr} t_{2} \xrightarrow{ww/wr} \dots \xrightarrow{ww/wr} t_{k} \xrightarrow{rw} t_1$ be the cycle in $DSG(H)$.
	
	Now we prove that $t_1 \in \dependsmath{e}{t_k}$ by induction:
	\begin{description}
		\item[Base case] We want to prove that $t_1 \in \dependsmath{e}{t_2}$.
		\begin{enumerate}
			\item If $t_1 \xrightarrow{ww} t_{2}$, there exists $k$ that $k \in \mathcal{W}_{t_1}$ and $k \in \mathcal{W}_{t_2}$, therefore $\mathcal{W}_{t_1} \cap \mathcal{W}_{t_2} \neq \emptyset $. 
			As proved above, $T_i\xrightarrow{ww}T_j \Rightarrow s_{T_i} \xrightarrow{*} s_{T_j}$, therefore we have $s_{t_1} \xrightarrow{*} s_{t_2}$. Therefore by definition, $t_1 \in \ddependsmath{e}{t_2}$. 
			
			\item If $t_1 \xrightarrow{wr} t_{2}$, there exists $o = r_2(x_1)$ that $t_2$ reads a version of $x$ $t1$ created.
			As proved above, $T_i\xrightarrow{wr}T_j \Rightarrow s_{T_i} \xrightarrow{+} s_{T_j}$, therefore we have $s_{t_1} \xrightarrow{+} s_{t_2}$. 
			Therefore $\sfomath{o}$ exists and $\sfomath{o} = s_{t_1}$, i.e. $t_1 = t_{\sfomath{o}}$.
			By definition, $t_1 \in \ddependsmath{e}{t_2}$. 
		\end{enumerate}
		
		Since $\ddependsmath{e}{t_2} \subseteq \dependsmath{e}{t_2}$, therefore $t_1 \in \dependsmath{e}{t_2}$.
		
		\item[Induction step] Assume $t_1 \in \dependsmath{e}{t_i}$, now we want to prove that $t_1 \in \dependsmath{e}{t_{i+1}}$.
		
		We first consider $t_i, t_{i+1}$, following the same analysis as in the base case, we have $t_{i} \in $ \\  $\ddependsmath{e}{t_{i+1}}$. Therefore $\dependsmath{e}{t_{i}} \subseteq \dependsmath{e}{t_{i+1}}$, we have $t_1 \in \dependsmath{e}{t_{i+1}}$.
		
	\end{description}
	
	Therefore we proved that $t_1 \in \dependsmath{e}{t_k}$.
	
	Since $t_k \xrightarrow{rw} t_1$, there exists $x$ such that $r_k(x_m) \in \Sigma_{t_k}$, $w_1(x_1) \in \Sigma_{t_1}$ and $x_m << x_1$. 
	Therefore we have $t_1 \in \dependsmath{e}{t_k}$, $r_k(x_m) \in \Sigma_{t_k}$ and $r_k(x_m).k \in \mathcal{W}_{t_1}$.
	Since $e$ satisfies $\forall t \in \mathcal{T}:\commitmath{PSI}{t}{e}$, we have $s_{t_1} \xrightarrow{*} \slomath{r_k(x_m)}$. 
	
	However, from $x_m << x_1$, we have $\forall s, s', s.t. (x,x_m) \in s \wedge (x,x_1) \in s' \Rightarrow s \xrightarrow{+} s'$. Since $(x,x_m) \in \slomath{r_k(x_m)} \wedge (x,x_1) \in s_{t_1}$, we have $\slomath{r_k(x_m)} \xrightarrow{+} s_{t_1}$. This contradicts with $s_{t_1} \xrightarrow{*} \slomath{r_k(x_m)}$, therefore we have proved \textit{H} does not exhibit
	phenomenon $G\text{-single}$, i.e. $\exists e:\forall t \in \mathcal{T}:\commitmath{PSI}{t}{e} \Rightarrow \lnot G1 \land \lnot G\text{-single}$.
	
	($\Leftarrow$) Now we prove the other direction $\lnot G1 \land \lnot G\text{-single} \Rightarrow \exists e:\forall t \in \mathcal{T}:\commitmath{PSI}{t}{e}$, 
	
	$\lnot G1 \land \lnot G\text{-single} \Rightarrow \exists e:\forall t \in \mathcal{T}:   \prereadmath{e}{t} \wedge \forall o \in \Sigma_t: \forall t' \in \dependsmath{e}{t}: o.k \in \mathcal{W}_{t'} \Rightarrow s_{t'} \xrightarrow{*} sl_o$
	
	We construct $e$ as follows: Consider only dependency edges in the DSG(H), by $\lnot G1$, there's no cycle consists of only dependency edges, therefore the transactions can be topologically sorted respecting only dependency edges. Let $i_1,...i_n$ be a permutation of $1,2,...,n$ such that $t_{i_1},...,t_{i_n}$ is a topological sort of DSG(H) with only dependency edges. We construct an execution $e$ according to the topological order defined above: $e: s_0 \rightarrow s_{t_{i_1}}\rightarrow s_{t_{i_2}} \rightarrow ... \rightarrow s_{t_{i_n}}$. 
	
	First we prove that $\prereadmath{e}{t}$ is true.
	
	Since the topological order consists with $wr$ edges, therefore for any $t_i \xrightarrow{wr} t_j$, we know that $t_i$ is applied before $t_j$, i.e. $s_{t_i} \xrightarrow{*} s_{t_j}$, then for any $o=r(k,v) \in \Sigma_{t}$,  $s_{t_i} \in \RSmath{o}$, therefore $\RSmath{o} \neq \emptyset$. Hence we have $\prereadmath{e}{t}$ is true.
	
	Now we prove that $\forall o \in \Sigma_t: \forall t' \in \dependsmath{e}{t}: o.k \in \mathcal{W}_{t'} \Rightarrow s_{t'} \xrightarrow{*} sl_o$ is also true.
	
	For any $t' \in \dependsmath{e}{t}$, by Lemma~\ref{lemma:predtrans}, $s_{t'} \xrightarrow{+}s_t$. Consider any $o \in \Sigma_t$, let $t'$ be a transaction that $t' \in \dependsmath{e}{t} \wedge o.k \in \mathcal{t'}$, we now prove that $s_{t'} \xrightarrow{*} sl_o$.
	
	
	Consider the three possible types of operations in $t$: 
	\begin{enumerate}
		\item \textit{External Reads}: an operation reads an object version
		that was created by another transaction. 
		\item \textit{Internal Reads}: an operation reads an object version that
		itself created.
		\item \textit{Writes}: an operation creates a new object version. 
	\end{enumerate}
	We show that $s_{t'} \xrightarrow{*} sl_o$ in each of those operation types:
	\begin{enumerate}
		\item \textit{External Reads}. Let $o=r(x_{\hat{t}})\in \Sigma_t$  read the
		version for $x$ created by $\hat{t}$, where $\hat{t} \neq t$. Since $\prereadmath{e}{t}$ is true, we have $\RSmath{o} \neq \emptyset$, therefore $s_{\hat{t}} \xrightarrow{+} s_t$ and $\hat{t}= t_{\sfomath{o}}$. From $\hat{t}= t_{\sfomath{o}}$, we have $\hat{t} \in \ddependsmath{e}{t}$.
		
		Now consider $t'$ and $\hat{t}$, we have proved that $s_{t'} \xrightarrow{+}s_t$ and $s_{\hat{t}} \xrightarrow{+} s_t$. Therefore there are two cases:
		
		\begin{itemize}
			\item $s_{t'} \xrightarrow{*} s_{\hat{t}}$: Given this, we have $s_{t'} \xrightarrow{*} s_{\hat{t}} =\sfomath{o} \xrightarrow{*} \slomath{o}$, therefore we have proved $s_{t'} \xrightarrow{*} \slomath{o}$.
			
			\item $s_{\hat{t}} \xrightarrow{+} s_{t'}$: Since $o.k \in \mathcal{W}_{t'}$, therefore $t'$ also write key $x_{t'}$, and since $s_{\hat{t}} \xrightarrow{+} s_{t'}$, by the way we assign the version order, we will have $x_{\hat{t}} << x_{t'}$, therefore there must be a chain of $ww$ edges between $\hat{t}$ and $t'$ in $DSG(H)$, where all of the transactions on the chain writes a new version of key $x$. Now consider the transaction on the chain directly next to $\hat{t}$, denoted as $\hat{t}_{+1}$, therefore we know that $\hat{t} \xrightarrow{ww} \hat{t}_{+1} \xrightarrow{ww}^* t'$. Note that $\hat{t}_{+1}$ overwrites the version of $x$ $t$ reads, therefore $t$ directly anti-depends $\hat{t}_{+1}$, i.e. $t \xrightarrow{rw}\hat{t}_{+1}$. Since $t' \in \dependsmath{e}{t}$, by Lemma~\ref{lemma:predchain},  we have $t' \xrightarrow{ww/wr}^+ t$. Now we claim there is a cycle consists of only one anti dependency edges as $t \xrightarrow{rw} \hat{t}_{+1} \xrightarrow{ww}^* t' \xrightarrow{ww/wr}^+ t$, which contradicts with $G\text{-single}$. Therefore this case cannot happen.
		\end{itemize}
		
		Therefore we proved that only $s_{t'} \xrightarrow{*} s_{\hat{t}}$ can happen, therefore we had the conclusion that $s_{t'} \xrightarrow{*} \slomath{o}$.
		
		\item \textit{Internal Reads}. Let $o=r(x_t)$
		read $x_t$ such that $w(x_t)\xrightarrow{to}r(x_t)$. By definition of $\RSmath{o}$, we have $\slomath{o} = s_p(t)$. Since we have proved that $s_{t'} \xrightarrow{+} s_t$, therefore we have $s_{t'} \xrightarrow{*} s_p(t) = \slomath{o}$.
		
		\item \textit{Writes}.  Let $o=w(x_t)$ be a write operation. By definition of $\RSmath{o}$, we have $\slomath{o} = s_p(t)$. Since we have proved that $s_{t'} \xrightarrow{+} s_t$, therefore we have $s_{t'} \xrightarrow{*} s_p(t) = \slomath{o}$.
	\end{enumerate}

	Therefore we proved that $\forall o \in \Sigma_t: \forall t' \in \dependsmath{e}{t}: o.k \in \mathcal{W}_{t'} \Rightarrow s_{t'} \xrightarrow{*} sl_o$ is true.
	\[
	\ddependsmath{e}{\hat{t}}=
	\{t| \exists o \in \Sigma_{\hat{t}}, t=t_{{sf_o}}\}
	\cup \{t|s_{t} \xrightarrow{+} s_{\hat{t}} \wedge \mathcal{W}_{\hat{t}} \cap \mathcal{W}_{t} \neq \emptyset \}\]
	\[
	\dependsmath{e}{\hat{t}} = (\bigcup_{t \in \ddependsmath{e}{\hat{t}}} \dependsmath{e}{t} )\cup \ddependsmath{e}{\hat{t}}
	\]
	\[
	\commitmath{PSI}{t}{e} \equiv \prereadmath{e}{t} \wedge \forall o \in \Sigma_t: \forall t' \in \dependsmath{e}{t}: o.k \in \mathcal{W}_{t'} \Rightarrow s_{t'} \xrightarrow{*} sl_o
	\]
	
	
\end{proof}







\subsection{Gotsman et al.'s model}
Gotsman consider a database storing objects $Obj = \{x, y, . . .\}$., and the set of operations as $Op = \{read(x, n), write(x, n) | x \in Obj, n \in \mathbb{Z}\}$, where Gotsman assumes the value space to be $\mathbb{Z}$ for simplicity. 

History events are of the form $(\iota, op)$, where $\iota$ is an identifier from a countably infinit set EventId and $op \in Op$. Let $WEvent_x =\{(\iota, write(x, n)) | \iota \in EventId, n \in  \mathbb{Z}\}$, 
$REvent_x =\{(\iota, write(x, n)) | \iota \in EventId, n \in  \mathbb{Z}\}$, and $HEvent_{x} = REvent_{x} \cap WEvent_{x}$. 
\begin{definition}
	A transaction $T$ is a pair $(E, po)$, where $E \subseteq HEvent$ is an
	non-empty set of events with distinct identifiers, and the program order $po$ is a total order over $E$. A history $\mathcal{H}$ is a set of transactions with disjoint sets of event identifiers.
\end{definition} 

\begin{definition}
	An abstract execution is a triple $A = (\mathcal{H}, VIS, AR)$ where:
	visibility $VIS \subseteq \mathcal{H} \times \mathcal{H} $is an acyclic relation; and
	arbitration $AR \subseteq \mathcal{H} \times \mathcal{H} $ is a total order such that $AR \supseteq VIS$.
\end{definition}

 \begin{definition}
 	Notations:
 	\begin{description}
 		
 		\item[$\_$]: Denotes a value that is irrelevant and implicitly existentially quantified.
 		
 		\item[$\max_R(A)$]: Given a total order $R$ and a set $A$, $\max_R(A)$ is the element $u \in A$ such that $\forall v \in A. v = u \vee (v, u) \in R$. 
 		
 		\item[$R_{-1} (u)$]: 
 		For a relation $R \subseteq A \times A$ and
 		an element $u \in A$, we let $R_{−1} (u) = \{v | (v, u) \in R\}$. 
 		\item[$T\vdash Write\ x:n$] $T$ writes to $x$ and
 		the last value written is $n$: $\max_{po}(E \cap WEvent_{x}) = (\_, write(x, n))$.
 		
 		\item[$T\vdash Read\ x:n$]: $T$ makes an external read from $x$, i.e., one before writing to $x$, and $n$ is the value returned by the first such read: $\min_{po}(E \cap HEvent_{x}) = (\_, read(x, n))$.
 	
 	\end{description}
 \end{definition}

 
\begin{definition}
	Consistency axioms:
	\begin{description}
		 \item[INT] $\forall(E,po) \in \mathcal{H}. \forall event \in E. \forall x,n. (event = (\_,read(x,n))\wedge (po^{-1}(event)\cap \textit{HEvent}_x \neq \emptyset))$\\ $\Rightarrow \max_{po}(po^{-1}(event)\cap \textit{HEvent}_x)=(\_,\_(x,n))$
		 
		 \item[EXT] 	$\forall T \in \mathcal{H}.\forall x,n. T \vdash Read\ x:n \Rightarrow$
		 $((VIS^{-1}(T)\cap\{S| S \vdash Write\ x:\_\} = \emptyset \wedge n = 0) \vee$\\
		 $ \max_{AR}((VIS^{-1}(T) \cap\{S| S \vdash Write\ x:\_\}) \vdash Write\ x:n)$
		 
		 \item[TRANSVIS] VIS is transitive
		 \item[NOCONFLICT] $\forall T,S \in \mathcal{H}. (T \neq S \wedge T \vdash Write x:\_ \wedge S \vdash Write x: \_) \Rightarrow (T\xrightarrow{VIS} S \vee S \xrightarrow{VIS} T)$
	\end{description}
\end{definition}

\begin{definition}
	PSI allows histories for which there exists an execution that satisfies INT, EXT,TRANSVIS and NOCONFLICT:
	$Hist_{PSI} = \{H | \exists VIS, AR.(\mathcal{H}, VIS, AR) \models$ {INT, EXT,TRANSVIS, NOCONFLICT}\}.
\end{definition}

\subsection{Equivalence}
\begin{theorem}
	Let $\mathcal{I}$ be PSI. Then $\exists e:\forall t \in \mathcal{T}:\commitmath{PSI}{t}{e} \equiv PSI_A$
\end{theorem}

\begin{proof}
	
	
	Transaction defined in Gotsman's model is slightly different from our model: Gotsman's transaction is a tuple of $(E,po)$, where $E$ is a set of events, and $po$ is the program order over $E$, whereas in our model a transaction is a tuple $(\Sigma_t, \xrightarrow{to})$, where $\Sigma_t$ is a set of operations, and $\xrightarrow{to}$ is the total order on $\Sigma_t$. Now that given a transaction, we denote it as $T$ in Gotsman's model, and $t$ in our model. We claim that $T$ and $t$ are equivalent if they represent the same transaction in two models. Event defined in Gotsman's model is a extension of an operation by attaching an unique identifier to an operation. Therefore we claim that a event in Gotsman's model is equivalent to an operation in our model if they represent the same operation.
	
	
($\Rightarrow$) First we prove the direction that $\exists e:\forall t \in \mathcal{T}:\commitmath{PSI}{t}{e} \Rightarrow PSI_A$.

Let $e$ be the execution that $\forall t \in \mathcal{T}:\commitmath{PSI}{t}{e}$.

$AR$ order is defined as $T_i \xrightarrow{AR} T_j \Leftrightarrow s_{t_i} \xrightarrow{} s_{t_j}$.
 And $VIS$ order is defined as $T_i \xrightarrow{VIS} T_j \Leftrightarrow t_i \in \dependsmath{e}{t_j}$.


\begin{description}
	\item[INT] 
	
	 $\forall(E,po) \in \mathcal{H}. \forall event \in E. \forall x,n. (event = (\_,read(x,n))\wedge (po^{-1}(event)\cap \textit{HEvent}_x \neq \emptyset))$\\ $\Rightarrow \max_{po}(po^{-1}(event)\cap \textit{HEvent}_x)=(\_,\_(x,n))$
	 
	 For any $(E,po) \in \mathcal{H}$, we consider any $event$ and $x$ that $(event = (\_,read(x,n))\wedge (po^{-1}(event)\cap \textit{HEvent}_x \neq \emptyset))$, we want to prove that $ \max_{po}(po^{-1}(event)\cap \textit{HEvent}_x)=(\_ ,\_ (x,n))$. Note that we denote the transaction $(E,po)$ as $T$ in Gotsman's model, and $t$ in our model.
	 
	 Since $(po^{-1}(event)\cap \textit{HEvent}_x \neq \emptyset))$, we have $\max_{po}(po^{-1}(event)\cap \textit{HEvent}_x)$ exists, and is either a read operation, or a write operation.
	 
	 \begin{enumerate}
	 	\item If $op = \max_{po}(po^{-1}(event)\cap \textit{HEvent}_x)$ is a write operation. Given that $event = (\_,read(x,n))$ and $op \xrightarrow{po} event$, therefore $event$ is a $read(x,n)$ in our model, and $op$ is a $w(x,v_{op})$ in our model, and $w(x,v_{op}) \xrightarrow{to} r(x,n)$, Since we required in our model that $w(k,v') \xrightarrow{to} r(k,v) \Rightarrow v = v'$, we have $v_{op} = n$, i.e. $op=(\_ , write(x,n))$, therefore $op = (\_ , \_ (x,n)$. 
	 	
	 	\item If $op=\max_{po}(po^{-1}(event)\cap \textit{HEvent}_x)$ is a read operation, let $op = (\_,read(x,v_{op}))$. Given $event = (\_,read(x,n))$ and $op \xrightarrow{po} event$, we have $event$ is equivalent to $ o_1 = r(x,n)$, $op$ is equivalent to $o_2 = r(x,v_{op})$ in our model, and $o_2 \xrightarrow{to} o_1$. Now we consider the following two cases.
	 	
	 	If there exists $w(k,v) \xrightarrow{to} o_2 \xrightarrow{to} o_1$, note that $ \xrightarrow{to}$ is a total order, we have$w(k,v) \xrightarrow{to} o_1$ and $w(k,v) \xrightarrow{to} o_2$ therefore by $w(k,v') \xrightarrow{to} r(k,v) \Rightarrow v = v'$, we have that $v = n \land v = v_{op}$, i.e. $v_{op} = n$.
	 	
	 	If there does not exist $w(k,v) \xrightarrow{to} o_2 \xrightarrow{to} o_1$. We prove by contradiction. Assume that $v_{op} \neq n$.
	 	We consider transaction $t_1$ that writes $(x,n)$, and $t_2$ that writes $(x,v_{op})$, by $\prereadmath{e}{\mathcal{T}}$ , we know $\sfomath{o_1}, \sfomath{o_2}$ exists, therefore we have $t_1 = t_{\sfomath{o_1}}$ and $t_2 = t_{\sfomath{o_2}}$, by definition of $\dependsmath{e}{t}$, we have $t_1,t_2 \in \ddependsmath{e}{t} \subseteq \dependsmath{e}{t}$, i.e. $t_1,t_2 \in \dependsmath{e}{t}$.
	 	
	 	Note that the sequence of states containing $(x,n)$ is disjoint from states contains $(x,v_{op})$, therefore either $s_{t_1} \xrightarrow{*} \slomath{o_1} \xrightarrow{+} s_{t_2} \xrightarrow{*} \slomath{o_2}$, or $s_{t_2} \xrightarrow{*} \slomath{o_2} \xrightarrow{+} s_{t_1} \xrightarrow{*} \slomath{o_1}$. Therefore we will have either $t_2 \in \dependsmath{e}{t} \wedge o_1.k \in \mathcal{W}_{t_2} \wedge \slomath{o_1} \xrightarrow{+} s_{t_2}$, or $t_1 \in \dependsmath{e}{t} \wedge o_2.k \in \mathcal{W}_{t_1} \wedge \slomath{o_2} \xrightarrow{+} s_{t_1}$; either case, it's a violation of $\commitmath{PSI}{t}{e}$, contradiction.
	 	Therefore the assumption cannot be true, hence we have $v_{op} = n$, i.e. $op=(\_ , read(x,n))$, therefore $op = (\_ , \_ (x,n)$. 
	 \end{enumerate}
	Therefore we proved that $ \max_{po}(po^{-1}(event)\cap \textit{HEvent}_x)=(\_ ,\_ (x,n))$.
	
	
	\item[EXT] 
	
	$\forall T \in \mathcal{H}.\forall x,n. T \vdash Read\ x:n \Rightarrow$
	$((VIS^{-1}(T)\cap\{S| S \vdash Write\ x:\_\} = \emptyset \wedge n = 0) \vee$\\
	$ \max_{AR}((VIS^{-1}(T) \cap\{S| S \vdash Write\ x:\_\}) \vdash Write\ x:n)$
	
	
	Consider any $T \in \mathcal{H}.\forall x,n. T \vdash Read\ x:n $, we have $T$ is equivalent to a transaction $t$ in our model, that $r(x,n) \in \Sigma_t$; since $T \vdash Read\ x:n $ denotes a external read of $T$, therefore $\not\exists w(x,n)\in \Sigma_t$.
	Let $t_n$ be the transaction that write $(x,n)$, and we know that $o=r(x,n) \in \Sigma_t$. By $\prereadmath{e}{\mathcal{T}}$, $t \in \mathcal{T}$ we have $\sfomath{o}$ exists and $\sfomath{o} = s_{t_n}$, i.e. $t_n = t_{\sfomath{o}}$. Therefore by definition of $\dependsmath{e}{t}$, we have $t_n \in \ddependsmath{e}{t} \subseteq \dependsmath{e}{t}$, i.e. $t_n \in \dependsmath{e}{t}$. 
	Since we defined VIS as $T_i \xrightarrow{VIS} T_j \Leftrightarrow t_i \in \dependsmath{e}{t_j}$, we have $T_n \xrightarrow{VIS} T$, therefore we have $T_n \in VIS^{-1}(T)$ and since $write(x,n) \in \Sigma_{t_n}$, $T_n \vdash Write\ x:n$.
	
	Now we argue that $T_n$ is larger in $AR$ order than any other $T'$, such that $T' \xrightarrow{VIS} T \wedge T' \vdash Write\ x:\_$. Consider the equivalent transaction $t'$ in our model, we know $t' \in \dependsmath{e}{t}$ and $x \in \mathcal{W}_{t'}$. Note that $o=r(x,n) \in \Sigma_t$, we will have $t' \in \dependsmath{e}{t} \wedge o.k \in \mathcal{W}_{t'} $, by $\commitmath{PSI}{t}{e} $, we have $s_{t'} \xrightarrow{*} \slomath{o}$. However since $t' \neq t_n$, we have $x_{t'} \neq n$. Note that $(x,x_{t'}) \in s_{t'}$, and $(x,n$) belongs to all the states that is between $\sfomath{o}$ and $\slomath{o}$, therefore we have $s_{t'} \xrightarrow{+}   \sfomath{o}=s_{t_n}$. Therefore we have $T' \xrightarrow{AR} T_n$, i.e. $T_n = \max_{AR}((VIS^{-1}(T) \cap\{S| S \vdash Write\ x:\_\})$. 
	
	Therefore we have proved that $\max_{AR}((VIS^{-1}(T) \cap\{S| S \vdash Write\ x:\_\})  \vdash Write\ x:n$.
	
	Therefore we have proved $\forall T \in \mathcal{H}.\forall x,n. T \vdash Read\ x:n \Rightarrow \max_{AR}((VIS^{-1}(T) \cap\{S| S \vdash Write\ x:\_\})  \vdash Write\ x:n$, EXT is true.
	
	\item[TRANSVIS] First we prove that $t_i \in \dependsmath{e}{t_j} \wedge t_j \in \dependsmath{e}{t_k} \Rightarrow t_i \in \dependsmath{e}{t_k}$. 
	
	We prove it by induction, let $e$ be $s_0 \rightarrow s_{t_1} \rightarrow s_{t_2} \rightarrow \dots \rightarrow s_{t_n}$:
	
	
	\begin{description}
		\item[Base case] 
		
		Consider the first transaction $t_1$ in the execution. We want to prove that for all transactions $t$ that precede $t_1$ in the execution
		$s_t \xrightarrow{*} s_{t_1} : \forall t' \in \dependsmath{e}{t}: s_{t'} \xrightarrow{*} s_{t}$. As $t_1$ is the first transaction in the execution, 
		$\ddependsmath{e}{t_1}=\emptyset$ and consequently $\dependsmath{e}{t} = \emptyset$. We see this by contradiction: assume there exists a transaction $t \in \ddependsmath{e}{t_1}$, by implication $s_t \xrightarrow{+} s_{t_1}$ (Lemma~\ref{lemma:preddirect}), violating
		our assumption that $t_1$ is the first transaction in the execution. Hence the desired result 
		trivially holds. 
		
		\item[Induction step] 
		Consider the i-th transaction in the execution. We assume that $\forall t \text{s.t.} s_t \xrightarrow{*} s_i$ the property $\forall t' \in \dependsmath{e}{t}: \dependsmath{e}{t'} \subseteq \dependsmath{e}{t}$ holds. In other words, we assume that the property holds
		for the first \textit{i} transactions. We now prove that the property holds for
		the first \textit{i+1} transactions, specifically, we show that $ \forall t' \in \dependsmath{e}{t_{i+1}}: \dependsmath{e}{t'} \subseteq \dependsmath{e}{t_{i+1}}$. A transaction $t'$ belongs to $\dependsmath{e}{t_{i+1}}$ if one of two conditions holds: either 
		$t' \in \ddependsmath{e}{t_{i+1}}$, or $ \exists t_k \in \mathcal{T}:t' \in \dependsmath{e}{t_k} \wedge t_k \in \ddependsmath{e}{t_{i+1}}$. We consider each in turn:
		
		\begin{itemize}
			\item If $t' \in \ddependsmath{e}{t_{i+1}}$: by definition of $\dependsmath{e}{t_{i+1}}$, $\dependsmath{e}{t'} \subseteq \dependsmath{e}{t_{i+1}}$.
			\item If $ \exists t_k \in \ddependsmath{e}{t_{i+1}}: t' \in \dependsmath{e}{t_k}$: As $t_k \in \ddependsmath{e}{t_{i+1}}$, by definition of $\dependsmath{e}{t_{i+1}}$, $\dependsmath{e}{t_k} \subseteq \dependsmath{e}{t_{i+1}}$
			The induction hypothesis holds for every transaction that precedes $t_{i+1}$ in $e$,
			hence $\forall t_{k'} \in \dependsmath{e}{t_k}: \dependsmath{e}{t_{k'}} \subseteq   \dependsmath{e}{t_k}$.
			As $t' \in \dependsmath{e}{t_k}$ by construction, it follows that $\dependsmath{e}{t'} \subseteq   \dependsmath{e}{t_k}$. Putting everything together, we have $\dependsmath{e}{t_{k'}} \subseteq   \dependsmath{e}{t_k} \subseteq \dependsmath{e}{t_{i+1}}$, and consequently $\dependsmath{e}{t_{k'}} \subseteq \dependsmath{e}{t_{i+1}}$. This completes the induction step of the proof.
		\end{itemize}
		
		Combining the base case, and induction step, we conclude:  $\forall t' \in \dependsmath{e}{t_{i+1}}: \dependsmath{e}{t'} \subseteq \dependsmath{e}{t_{i+1}}$.
	\end{description}
	
	Therefore if $T_i \xrightarrow{VIS} T_j \wedge T_j \xrightarrow{VIS} T_k$, we have $t_i \in \dependsmath{e}{t_j} \wedge t_j \in \dependsmath{e}{t_k}$. From $t_j \in \dependsmath{e}{t_k}$, by the induction, we know that $\dependsmath{e}{t_j} \subseteq \dependsmath{e}{t_k}$, therefore we have $t_i \in \dependsmath{e}{t_k}$. By how we defined $VIS$, we have $T_i \xrightarrow{VIS} T_k$., therefore we proved $VIS$ is transitive.
	
	\item[NOCONFLICT]
	$\forall T,S \in \mathcal{H}. (T \neq S \wedge T \vdash Write x:\_ \wedge S \vdash Write x: \_) \Rightarrow (T\xrightarrow{VIS} S \vee S \xrightarrow{VIS} T)$
	
	 Consider any $T,S \in \mathcal{H}. (T \neq S \wedge T \vdash Write x:\_ \wedge S \vdash Write x: \_) $, let $t_i, t_j$ be the transactions equivalent to $T,S$ respectively, we have $ x \in \mathcal{W}_{t_i} \cap \mathcal{W}_{t_j}$, let $w(x, x_i) \in \Sigma_{t_i}$ and $w(x, x_j) \in \Sigma_{t_j} $. 
	Since $e$ is a total order on all the committed transactions, we have either $s_{t_i} \xrightarrow{+} s_{t_j}$ or $s_{t_j} \xrightarrow{+} s_{t_i}$. 
	
	If $s_{t_i} \xrightarrow{+} s_{t_j}$,
	since $s_{t_i} \xrightarrow{+} s_{t_j} \wedge \mathcal{W}_{t_i} \cap \mathcal{W}_{t_j} \neq \emptyset$, we have $t_i \in \ddependsmath{e}{t_j} \subseteq \dependsmath{e}{t_j}$, i.e. $t_i \in  \dependsmath{e}{t_j}$, therefore we have $T \xrightarrow{VIS} S$.
	
	Similarly, if $s_{t_j} \xrightarrow{+} s_{t_i}$, 
	since $s_{t_j} \xrightarrow{+} s_{t_i} \wedge \mathcal{W}_{t_i} \cap \mathcal{W}_{t_j} \neq \emptyset$, we have $t_j \in \ddependsmath{e}{t_i} \subseteq \dependsmath{e}{t_i}$, i.e. $t_j \in  \dependsmath{e}{t_i}$, therefore we have $S \xrightarrow{VIS} T$.

	
	Therefore we proved that $T\xrightarrow{VIS} S \vee S \xrightarrow{VIS} T$, NOCONFLICT is true.
\end{description}


($\Leftarrow$) Now we prove the direction that $ PSI_A  \Rightarrow \exists e:\forall t \in \mathcal{T}:\commitmath{PSI}{t}{e}$.

Since AR is a total order over $\mathcal{T}$, we construct execution $e$ by applying transactions in the same order as AR, i.e. $s_{t_i} \xrightarrow{+} s_{t_j} \Leftrightarrow T_i \xrightarrow{AR} T_j$. Now we want to prove that $e$ satisfies $\forall t \in \mathcal{T}:\commitmath{PSI}{t}{e}$.



First we prove that $\prereadmath{e}{\mathcal{T}}$ is true: Consider any transaction $t$, for any operation $o \in \Sigma_t$, if $o$ is a internal read operation or $o$ is a write operation, then by definition $\sfomath{o} = s_0 \xrightarrow{*} s_t$ follows trivially. If $o$ is a read operation that reads a value written by another transaction $t'$: Consider $T$ in Gotsman's model corresponding to $t$, we have $T \vdash Read\ x:n$ and $T' \vdash Write\ x:n$. 
Since we assumed values are uniquely identifiable, we have $T'= \max_{AR}(VIS^{-1}(T) \cap\{S| S \vdash Write x:\_\})$ by EXT, therefore $T' \in VIS^{-1}(T)$, i.e. $t' \xrightarrow{VIS}t$, since $VIS \subseteq AR$, therefore $T' \xrightarrow{AR}T$. 
Note that we apply transactions in the same order as $AR$, we have $s_{t'} \xrightarrow{*} s_{t}$. 
Since we have $(x,n) \in s_{t'}$ and $s_{t'} \xrightarrow{*} s_{t}$, therefore $s_{t'} \in \RSmath{o}$, hence $\RSmath{o} \neq \emptyset$. We proved any transaction $t$, for any operation $o \in \Sigma_t$, $\RSmath{o} \neq \emptyset$, therefore $\prereadmath{e}{\mathcal{T}}$ is true.

Now consider any $t\ in \mathcal{T}$, we want to prove that $\forall o \in \Sigma_t: \forall t' \in \dependsmath{e}{t}: o.k \in \mathcal{W}_{t'} \Rightarrow s_{t'} \xrightarrow{*} sl_o$. 


First we prove that $\forall t' \in  \dependsmath{e}{t} \Rightarrow T'\xrightarrow{VIS} T$. 

Since we have proved that $\prereadmath{e}{\mathcal{T}}$ is true, by Lemma~\ref{lemma:predchain} we know that there is a chain $t' \xrightarrow{wr/ww}^+ t$. Consider any edge on the chain: $t_i \xrightarrow{ww/wr} t_j$:

\begin{enumerate}
	\item $t_i \xrightarrow{ww} t_j$: We have $T_i,T_j \in \mathcal{H}$ and $(T_i \neq T_j \wedge T_i \vdash Write\ x:\_ \wedge T_j \vdash Write\ x:\_)$, therefore by NOCONFLICT, we have $t_i \xrightarrow{VIS} t_j \vee t_j \xrightarrow{VIS} t_i$. However note that $s_{t_i} \xrightarrow{*} s_{t_j}$, we know that $t_i \xrightarrow{AR} t_j$, and since $VIS \subseteq AR$, we have $t_i \xrightarrow{VIS} t_j$.
	\item $t_i \xrightarrow{wr} t_j$: Note that $\bot$ is the initial value of a key in our model, while $0$ is the initial value in Gotsman's model, $\bot$ corresponding to $0$ in Gotsman's model. 
	Let $n$ be the value that $t_i$ writes and $t_j$ reads, and transaction cannot write empty value, i.e. $\bot$, to a key, therefore we have $T_j \vdash Read\ x:n $ and $n \neq 0$ in Gotsman's model, therefore by EXT, $ \max_{AR}(VIS^{-1}(T_j) \cap\{S| S \vdash Write\ x:\_\}) \vdash Write\ x:n$. 
	Since $T_i \vdash Write \ x:n$, therefore $T_i = \max_{AR}(VIS^{-1}(T_j) \cap\{S| S \vdash Write\ x:\_\})$, hence we have $T_i \in VIS^{-1}(T_j) $, i.e. $T_i \xrightarrow{VIS} T_j$.
\end{enumerate}

Now we consider the chain $t' \xrightarrow{wr/ww}^+ t$, and we have that $T' \xrightarrow{VIS}^+ T$, by TRANSVIS, we have $T' \xrightarrow{VIS} T$.

Now, consider any $o \in \Sigma_t$ that $o.k \in \mathcal{W}_{t'}$, let $o.k = x$, therefore $T' \vdash Write\ x:\_$. Since we have proved that $T' \xrightarrow{VIS} T$, we have $T' \in VIS^{-1}(T) \cap\{S| S \vdash Write\ x:\_\}$. Now we consider the following two cases.

If $o$ is an external read, and read the value $(x,\hat{x})$ written by $\hat{t}$, since transaction cannot write empty value, i.e. $\bot$, to a key, therefore we have $T \vdash Read\ x:\hat{x} $ and $\hat{x} \neq 0$ in Gotsman's model, therefore by EXT, $ \max_{AR}(VIS^{-1}(T_j) \cap\{S| S \vdash Write\ x:\_\}) \vdash Write\ x:\hat{x}$. 
Since $\hat{T}\vdash Write\ x:n$, we have $\hat{T} = \max_{AR}(VIS^{-1}(T_j) \cap\{S| S \vdash Write\ x:\_\})$
, therefore $T' \xrightarrow{AR} \hat{T}$ or $T'  =\hat{T}$. Note that we apply transactions in the same order as $AR$, therefore we have $s_{t'} \xrightarrow{+} s_{\hat{t}}$ or $s_{t'} = s_{\hat{t}}$, i.e. $s_{t'} \xrightarrow{*}s_{\hat{t}}$. 
Since we proved that $\prereadmath{e}{t}$ is true, we have $\sfomath{o}$ exists and $s_{\hat{t}} = \sfomath{o}$, note that by definition $\sfomath{o} \xrightarrow{*} \slomath{o}$. Now we have $s_{t'}\xrightarrow{*} s_{\hat{t}}=\sfomath{o}\xrightarrow{*} \slomath{o}$, therefore $s_{t'} \xrightarrow{*} \slomath{o}$  . 

If $o$ is an internal read operation or write operation, then $\slomath{o} = s_p(t)$. Since $t' \in \dependsmath{e}{t}$, by Lemma~\ref{lemma:predtrans}, we have $s_{t'} \xrightarrow{+} s_{t}$, therefore $s_{t'} \xrightarrow{*} s_p({t}) = \slomath{o}$, i.e. $s_{t'} \xrightarrow{*} \slomath{o}$.

Therefore we proved that $\forall o \in \Sigma_t: \forall t' \in \dependsmath{e}{t}: o.k \in \mathcal{W}_{t'} \Rightarrow s_{t'} \xrightarrow{*} sl_o$. 

Now, we have proved that $e$ satisfies for any $t \in \mathcal{T}$, $\prereadmath{e}{\mathcal{T}} \wedge \forall o \in \Sigma_t: \forall t' \in \dependsmath{e}{t}: o.k \in \mathcal{W}_{t'} \Rightarrow s_{t'} \xrightarrow{*} sl_o$, i.e. $\forall t \in \mathcal{T}:\commitmath{PSI}{t}{e}$, therefore we proved that $\exists e:\forall t \in \mathcal{T}:\commitmath{PSI}{t}{e}$.

%Therefore $\hat{t} \xrightarrow{AR}t$. 










\end{proof}


==> readcommit.tex <==
\subsection{Read Committed}
\label{appendix:rc}
\par \textbf{Theorem ~\ref{theorem:rc}}. Let $\mathcal{I}$ be Read Committed (RC). Then $\ \ \exists e:\forall t
  \in \mathcal{T}. \commitmath{RC}{t}{e}  \equiv \lnot \gone $.

\begin{proof}
	  \textbf{We first prove} $\lnot \gone  \Rightarrow \exists e: \forall t \in \mathcal{T}: \commitmath{RC}{t}{e}$. 
	
Let $H$ define a history over $\mathcal{T}=\{t_1, t_2, ..., t_n\}$
and let $DSG(H)$ be the corresponding direct serialization graph.
 $\lnot \gonec$ states that the $DSG(H)$ must not contain dependency cycles:
 the subgraph of $DSG(H)$, $SDSG(H)$ containing the same nodes but
 including only dependency edges,  must be acyclic. Let $i_1,...i_n$ be a permutation of $1,2,...,n$ such that $t_{i_1},...,t_{i_n}$ is a topological sort of $SDSG(H)$ ($SDSG(H)$ is acyclic and can thus be topologically sorted).

 We construct an execution $e$ according to the topological order defined above: $e: s_0 \rightarrow s_{t_{i_1}}\rightarrow s_{t_{i_2}} \rightarrow ... \rightarrow s_{t_{i_n}}$ and show that $\forall t
  \in \mathcal{T}. \commitmath{RC}{t}{e}$. Specifically, we show that for
  all $t = t_{i_j}, \prereadmath{e}{t}$.
	
Consider the three possible types of operations in $t_{i_j}$: 
\begin{enumerate}
\item \textit{External Reads}: an operation reads an object version
that was created by another transaction. 
\item \textit{Internal Reads}: an operation reads an object version that
itself created.
\item \textit{Writes}: an operation creates a new object version. 
\end{enumerate}
We show that the parent state of $t_{i_j}$ is included in the read set of
each of those operation types:
\begin{enumerate}
		\item \textit{External Reads}. Let $r_{i_j}(x_{i_k})$  read the
        version for $x$ created by $t_{i_k}$, where $k \neq j$.\\ \\
We first show that $s_{t_{i_k}} \xrightarrow[]{*}  s_{t_{i_j}}$.
As $t_{i_j}$ directly read-depends on $t_{i_k}$, there must exist an edge $t_{i_k}\xrightarrow{wr}t_{i_j}$ in $SDSG(H)$, and  $t_{i_k}$ must
therefore be ordered before $t_{i_j}$ in the topological sort of $DSG(H)$ ($k<j$), it follows that  $s_{t_{i_k}} \xrightarrow[]{+}  s_{t_{i_j}}$. 
As $(x,x_{i_k}) \in s_{t_{i_k}}$, we have $s_{t_{i_{k}}} \in \RSmath{r_{i_j}(x_{i_k})}$, and consequently $\RSmath{r_{i_j}(x_{i_k})} \neq \emptyset$.
		
		\item \textit{Internal Reads}. Let $r_{i_j}(x_{i_j})$
        read $x_{i_j}$ such that $w(x_{i_j})\xrightarrow{to}r(x_{i_j})$. By definition, the read state set of such an operation consists
        of $\forall s \in \mathcal{S}_e: s\xrightarrow{*} s_p$.  $ s_0 \xrightarrow{*} s$ trivially holds. We conclude $s_0 \in \RSmath{r_{i_j}(x_{i_j})}$, i.e. $\RSmath{r_{i_j}(x_{i_j})} \neq \emptyset$. 
		\item \textit{Writes}.  Let $w_{i_j}(x_{i_j})$ be a write operation. By definition, its read state set consists of all the states before $s_{t_{i_{j}}}$ in
        the execution. Hence $s_0 \in \RSmath{r_{i_j}(x_{i_j})}$, i.e. $\RSmath{r_{i_j}(x_{i_j})} \neq \emptyset$. 
	\end{enumerate}
	
	Thus $\forall o \in \Sigma_t: \RSmath{o} \neq \emptyset$. We have $\prereadmath{e}{t_{i_j}}$ for any $t_{i_j}: \forall t \in \mathcal{T}: \commitmath{RC}{t}{e}$.
	
	
	($\Leftarrow$) \textbf{We next prove} $\exists e: \forall t \in
          \mathcal{T}: \commitmath{RC}{t}{e} \Rightarrow  \lnot \gone
        $.

To do so, we prove the contrapositive $\gone \Rightarrow \forall e\ \exists t \in \mathcal{T}: \lnot\commitmath{RC}{t}{e}$. Let $H$ be a history that displays phenomena \gone. We generate a contradiction. Assume that there exists an execution
$e$ such that $\forall t \in \mathcal{T}: \commitmath{RC}{t}{e}$. 

We first instantiate the version order for $H$, denoted as $<<$, as follows: given an execution $e$ and an object $x$, $ x_i << x_j$ if and only if $x \in \mathcal{W}_{t_i} \cap \mathcal{W}_{t_j} \land  s_{t_{i}} \xrightarrow{+} s_{t_{j}} $.
	
First, we show that: 	
	\begin{clm}
		$t_i \rightarrow t_j$ in $SDSG(H) \Rightarrow s_{t_i} \xrightarrow{*} s_{t_j}$ in the execution e ($i\neq j$).
		\label{ser1}
	\end{clm}
	\begin{proof}
		Consider the three edge types in $DSG(H)$:
		\begin{description}
			\item{$t_i\xrightarrow{ww}t_j$} There exists an object $x$ s.t. $x_i<<x_j$ (version order). 
By construction, we have $s_{t_i} \xrightarrow{+} s_{t_j}$.
			
			\item{$t_i\xrightarrow{wr}t_j$} There exists an object $x$ s.t. $t_j$ reads version 
            $x_i$ written by $t_i$, i.e. $r_j(x,x_i) \in \Sigma_{t_i}$. By assumption $\commitmath{RC}{e}{{t}}$ ($t=t_j$), i.e. $\prereadmath{e}{t_j}$, $\RSmath{o} \neq \emptyset$. Let $s \in \RSmath{o}$, by definition of $\RSmath{o}$, we have $(x,x_i) \in s \wedge s \xrightarrow{+} s_{t_j}$, therefore $t_i$ must be applied before or on state $s$, hence we have $s_{t_i}\xrightarrow{*} s \xrightarrow{+} s_{t_j}$, i.e. $s_{t_i} \xrightarrow{+} s_{t_j}$. 
			
		\end{description}
		
	\end{proof}

We now derive a contradiction in all cases of $\gone$: 
\begin{itemize}
\item Let us assume that $H$ exhibits
phenomenon \gonea~(aborted reads). There
must exists events $w_i(x_i), r_j(x_i)$ in
H such that $t_i$ subsequently aborted. $\mathcal{T}$ and any corresponding execution $e$, however, consists only of committed
transactions. Hence $\forall e: \not\exists s \in \mathcal{S}_e, s.t.\ s \in \RSmath{ r_j(x_i)}$: no
complete state can exists for $t_j$. There thus
exists a transaction for which the commit test cannot be satisfied, for any e. We have a contradiction.
\item  Let us assume that $H$ exhibits 
phenomenon \goneb~(intermediate reads). In an execution $e$, only the final writes of a transaction are applied. Hence,$\not\exists s \in \mathcal{S}_e, s.t.\ s \in \RSmath{ r(x_{intermediate})}$. There
thus exists a transaction, which for all e, will not 
satisfy the commit test. We once again have a contradiction.
		\item Finally, let us assume that the history $H$ displays \gonec. 
Any history that displays \gonec will contain a cycle in the SDSG(H). Hence, there must exist a chain of transactions $t_i\rightarrow t_{i+1} \rightarrow ... \rightarrow t_{j}$ such that $i=j$.
By Claim~\ref{ser1}, we thus have $s_{t_i} \xrightarrow{+} s_{t_{i+1}} \xrightarrow{+} \dots \xrightarrow{+} s_{t_j}$, $i=j$ for any $e$. By definition however, a valid execution must be totally ordered. We have our
final contradiction.
\end{itemize}
All cases generate a contradiction. We have
$\gone \Rightarrow \forall e: \exists t \in \mathcal{T}: \lnot\commitmath{RC}{e}{t}$. This
completes the proof. 
\end{proof}

